TrustAL: Trustworthy Active Learning using Knowledge Distillation

Active learning can be defined as iterations of data labeling, model training, and data acquisition, until sufficient labels are acquired. A traditional view of data acquisition is that, through iterations, knowledge from human labels and models is implicitly distilled to monotonically increase the accuracy and label consistency. Under this assumption, the most recently trained model is a good surrogate for the current labeled data, from which data acquisition is requested based on uncertainty/diversity. Our contribution is debunking this myth and proposing a new objective for distillation. First, we found example forgetting, which indicates the loss of knowledge learned across iterations. Second, for this reason, the last model is no longer the best teacher -- For mitigating such forgotten knowledge, we select one of its predecessor models as a teacher, by our proposed notion of "consistency". We show that this novel distillation is distinctive in the following three aspects; First, consistency ensures to avoid forgetting labels. Second, consistency improves both uncertainty/diversity of labeled data. Lastly, consistency redeems defective labels produced by human annotators.

==> backups/0_abstract.tex <==
\begin{abstract}
Active learning can be defined as iterations of data labeling, model training, and data acquisition, until sufficient labels are acquired. A traditional view of data acquisition is that, through iterations, knowledge from human labels and models is implicitly distilled to monotonically increase the accuracy and label consistency. Under this assumption, the most recently trained model is a good surrogate for the current labeled data, from which data acquisition is requested based on uncertainty/diversity. Our contribution is debunking this myth and proposing a new objective for distillation. First, we found example forgetting, which indicates the loss of knowledge learned across iterations. Second, for this reason, the last model is no longer the best teacher-- For mitigating such forgotten knowledge, we select one of its predecessor models as a teacher, by our proposed notion of ``consistency''. We show that this novel distillation is distinctive in the following three aspects; First, consistency ensures to avoid forgetting labels. Second, consistency improves both uncertainty/diversity of labeled data. Lastly, consistency redeems defective labels produced by human annotators.
\end{abstract}


%Active learning goes through an iterative process of labeling data, and each iteration is believed to be ``consistent'' from before, such that the most recently trained model is a good surrogate for the current labeled data. In this work, our main contribution is to debunk this myth by observing example forgetting which indicates the loss of knowledge learned across iterations. For this reason, we present TrustAL, a simple yet effective framework of mitigating such forgotten knowledge, which can be easily applied to existing active learning methods focusing on data acquisition. Specifically, when a new model is trained per iteration, we select one of its predecessor models as a teacher, and pass the knowledge to the new model via knowledge distillation. Therefore, the new model is a more trustworthy model itself, and simultaneously, yields better next data acquisition, consistently keeping the learned knowledge. Our extensive experiments show that TrustAL consistently outperforms baselines including state-of-the-art on three popular text classification datasets.


==> backups/1_backup_aug29.tex <==
\section{Introduction} \label{sec:intro}


%진영 20210822 오스태클 논문이 논지가 비슷하지 최대한 많이 활용

Labeling data is a fundamental bottleneck in machine learning due to annotation cost and time. One practical solution is Active Learning (AL): given a limited labeling budget $k$, which example should I ask human annotators to label?  Generally, this can be done over multiple generations of data acquisition and labeling, until sufficient labels are obtained. At each iteration, unlabeled yet the $k$ most desirable examples are recognized by the last trained model (\ie, data acquisition model) and added to the labeled dataset with the human labels to train a new model. That is, AL can be viewed as an \emph{iterative} process of data acquisition and model training, \emph{interacting with machine and human} in the iteration.

% what -> .... -> distillation  전환이 문제 
While a wide range of studies focus on ``how'' to identify valuable samples, \eg, uncertainty- or diversity-based~\cite{dasgupta2011two,xu2003representative,hu2010off,bodo2011active,ash2019deep} when given an acquisition model, there is little attention on ``what'' is proper for the acquisition model. A naive belief is that the latest model is a good reference or surrogate for the distribution of whole dataset or at least the currently labeled data such that the latest model works as an effective acquisition model for identifying informative samples. To validate such monotonic assumption, we analyze its knowledge-preserving ability by adopting correct-consistency~\cite{wang2020wisdom} as a measure. We hypothesize that the desirable acquisition model should preserve the valuable knowledge learned from the labels. In other words, correct prediction would be ``consistently'' kept across AL cycles. We evaluate such consistent behaviors of the trained models in development set, whether sample $i$ predicted correctly at iteration $t$ remains with the correct prediction at $t+1$, which is correct-consistency~\cite{wang2020wisdom}.% (which we call consistency for brevity).


Unfortunately, our empirical observation of inconsistency (reverse phenomenon of correct-consistency) called \emph{example forgetting}~\cite{toneva2018empirical} dispels the myth aforementioned. Specifically, it demonstrates that knowledge learned at some time from labeled dataset is suddenly forgotten across subsequent acquisition procedure. We argue that such loss of knowledge implies the ineligibility of the recent model to be treated as a good reference for labeled dataset. Such discrepancy between the labeled data and its referent acquisition model leads to wasting previous/subsequent labeling efforts by deteriorating the quality of data.



% Such monotonic assumption requires that the model knowledge learned from the labels is consistently kept across AL cycles. 

%That is, sample $i$ labeled correctly at iteration $t$ should remain with the correct label at $t+1$, which is correct-consistency~\cite{wang2020wisdom} between $t$ and $t+1$ (which we call consistency for brevity).
% When consistency holds for all items at any arbitrary $t$, the optimal AL strategy, such as diversity- or uncertainty-based~\cite{sener2017active,wang2014new}, is adopting data acquisition conditioned on the most recently trained model.

 %Here, we argue that it is critical to consider not only accuracy but also consistency for learning the trustworthy models during AL cycles.







Motivated by the above, in this paper, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), of bridging the knowledge discrepancy between labeled data and model. In TrustAL, our key idea is leveraging knowledge distillation~\cite{furlanello2018born}, which is orthogonally applicable to state-of-the-art AL methods~\cite{ash2019deep} focusing on data acquisition, in a synergistic manner.
Specifically, at each iteration, TrustAL searches for an expert predecessor model for the forgotten knowledge from a number of alternatives, then transfers the model knowledge (\eg, pseudo labels) to the current model training. By optimizing the dual goals of following not only oracle labels but also pseudo (soft) labels of a selected predecessor model, the newly trained model can relieve example forgetting events, and thus be the trustworthy surrogate for the next data acquisition. For this purpose, here we formalize the teacher selection problem across AL cycles: which predecessor is the most desired teacher for the forgotten knowledge? To resolve this, we present two teacher selection strategies, (1) monotonic choice of the most recent model (\ie, a proxy of the most accurate model), and (2) non-monotonic choice of the well-balanced model with accuracy and consistency. 

% 여기 더 적어야할지도.

%Specifically, we present two teacher selection strategies: (i) monotonic choice of using the most recently trained model (\ie, a proxy of the most accurate model), and (ii) non-monotonic choice of using the well-balanced model with both accuracy and consistency. 


Our experiments show that TrustAL significantly improves performance with various data acquisition methods while preserving the valuable knowledge from the labeled dataset. We validate pseudo labels from the predecessor model are not just approximate/weak predictions \text{-} It can be viewed as knowledge from the previous generation, and can be used as consistency regularization for conventional AL methods solely aiming at higher accuracy. 

==> backups/1_intro.tex <==
% issue list
% 1. trustworthy 가 뭔지 우리식으로 정의해야 할수도 있음(우리가 지적하는 세가지를 해결하면 trustworthy하다) (황승원 교수님 의견)

\section{Introduction} \label{sec:intro}

Labeling data is a fundamental bottleneck in machine learning due to annotation cost and time. One practical solution is Active Learning (AL): given a limited labeling budget $k$, which example should I ask human annotators to label?  Generally, this can be done through an \emph{iterative} process of labeling data, model training, and data acquisition steps, until sufficient labels are obtained. At each iteration, based on the last trained model, unlabeled yet the $k$ most desirable examples are recognized and added to the labeled dataset to train a new model. This process continues to the next iteration for selecting next $k$ unlabeled examples based on the newly trained model. That is, a naive belief in AL is that the last trained model can be a good reference or surrogate for the distribution of the currently labeled data, which indicates what examples are desired for the next model update.


In this work, our empirical observation dispels this myth. Although the model knowledge learned from the labels is expected to be ``consistently'' kept or improved across AL iterations, we find that knowledge learned at some time is suddenly forgotten, which indicates that the recent model is ineligible to be treated as a good reference of the labeled dataset. More specifically, we can observe such inconsistent behaviors of the trained model during inference time, where sample $i$ predicted correctly at iteration $t$ is predicted incorrectly at iteration $t + \Delta t$, which is called \emph{example forgetting}~\cite{toneva2018empirical}. 


Motivated by this, in this work, we argue that \textbf{correct-consistency} (which we call consistency for brevity) should be an essential criterion, which is the model ability to make consistent correct predictions across successive AL generations for the same input~\cite{wang2020wisdom}. In the view of consistency, prior AL methods only focusing on data acquisition steps~\cite{dasgupta2011two,xu2003representative,bodo2011active,ash2019deep} are still sub-optimal since the three transitions among AL steps may suffer from following problems due to inconsistency (reverse phenomenon of consistency),  which we empirically analyze later:
\begin{itemize}
    \item \textbf{From labeling to model training:} Despite successful data acquisition, the subsequent labeling efforts can be negated by forgetting the learned knowledge later, which wastes annotation cost. We argue that consistency is key to make a label-efficient AL (Figure~\ref{fig:rq1-Trec}). 

    \item \textbf{From model training to data acquisition:} Inconsistent data acquisition models cannot serve as a good reference for the current data distribution, which leads to contaminating the next data acquisition step. Improving consistency may be synergetic to either uncertainty- or diversity-based acquisition strategies (Figure~\ref{fig:rq2}).

    \item \textbf{From data acquisition to labeling:} Human annotators who act as oracles are usually subject to accidental mislabeling~\cite{bouguelia2018agreeing} which degrades traditional AL methods. Learning to keep consistency enables to mitigate the confusion from the noisy labels (Figure~\ref{fig:noisy_label}).
\end{itemize}


To overcome these drawbacks and thus make all the three transitions in AL more trustworthy, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), for bridging the knowledge discrepancy between labeled data and model. In TrustAL, our key idea is to add a new step in the iterative process of AL to learn the forgotten knowledge, which is orthogonally applicable to state-of-the-art data acquisition strategies in a synergistic manner. Specifically, at each iteration, TrustAL first searches for an expert model for the forgotten knowledge among the predecessor models. Then, TrustAL transfers the model knowledge (\eg, logits) to the current model training step by leveraging the knowledge distillation technique~\cite{hinton2015distilling}. By optimizing the dual goals of following both human labels and machine labels of the expert predecessor, the newly trained model can relieve forgotten knowledge and thus be more consistent, keeping its correct predictions.
%the trustworthy surrogate for the next data acquisition. 


For the purpose of identifying which predecessor is the most desired teacher to relieve the forgotten knowledge, we further explore the teacher selection problem. To resolve this, we present two teacher selection strategies, (1) \textbf{TrustAL-MC}: monotonic choice of the most recent model (\ie, a proxy of the most accurate model), 
and (2) \textbf{TrustAL-NC}: non-monotonic choice of the well-balanced model with accuracy and consistency, which we thoroughly design as analysis/evaluation measures in this paper. 


% 
Our experiments show that the TrustAL framework significantly improves performance with various data acquisition strategies while preserving the valuable knowledge from the labeled dataset. We validate the pseudo labels from the predecessor models are not just approximate/weak predictions \text{-} It can be viewed as knowledge from the previous generation, and can be used as consistency regularization for conventional AL methods solely aiming at higher accuracy. 

==> backups/1_intro_backup.tex <==
\section{Introduction} \label{sec:intro}


Labeling data is a fundamental bottleneck in machine learning due to annotation cost and time.
One practical solution is Active Learning (AL): given a limited labeling budget $k$, which example should I ask human annotators to label? Generally, this can be done over multiple generations, until sufficient labels are obtained. At each iteration, based on the last trained model, unlabeled yet the $k$ most desirable examples are recognized and added to the labeled training set, and the process continues to the next iteration for selecting next $k$ unlabeled examples based on a newly trained model. That is, AL can be viewed as an \emph{iterative} process of data acquisition and model training.


This iterative process is based on a naive belief that the
last trained model can be a good reference or surrogate for the distribution of all prior iterations or the currently labeled data.
% data의 good reference = data의 knowledge를 잘 반영함이다
% 이걸 말해야 monotonic assumption이 성립한다는 말 = consistent(knowledge를 잘반영한다) 하다의 관계가 성립하는 거 같습니다.
Such an assumption requires that valuable knowledge learnt from the labels is ``consistently'' kept across AL cycles. For example, we can evaluate such consistent behaviors of the trained models in development set, where sample $i$ labeled correctly at iteration $t$ should remain with the correct label at $t+1$, which is correct-consistency~\cite{wang2020wisdom} between $t$ and $t+1$ (which we call consistency for brevity).
% 아래 문장이 어떤 뜻인지 이해가 잘 가지 않았습니다.
When the consistency holds for all items at any arbitrary $t$, the optimal data acquisition strategy, such as diversity- or uncertainty-based~\cite{sener2017active,wang2014new}, works better conditioned on the last trained model.

% Such monotonic assumption requires that the model knowledge learned from the labels is consistently kept across AL cycles. 

%That is, sample $i$ labeled correctly at iteration $t$ should remain with the correct label at $t+1$, which is correct-consistency~\cite{wang2020wisdom} between $t$ and $t+1$ (which we call consistency for brevity).
% When consistency holds for all items at any arbitrary $t$, the optimal AL strategy, such as diversity- or uncertainty-based~\cite{sener2017active,wang2014new}, is adopting data acquisition conditioned on the most recently trained model.



However, our empirical observation of inconsistency called \emph{example forgetting}~\cite{toneva2018empirical,wang2020wisdom} dispels this myth. Specifically, it demonstrates that knowledge learnt at some time from labeled dataset is suddenly forgotten across subsequent acquisition procedure. We argue that such loss of knowledge implies the ineligibility of the recent model to be treated as a good reference for labeled dataset. Such discrepancy between the labeled data and its untrustworthy surrogate leads to wasting labeling efforts by deteriorating the quality of data acquisition~\cite{prabhu2019sampling}. %Here, we argue that it is critical to consider not only accuracy but also consistency for learning the trustworthy models during AL cycles.







Motivated by the above, in this paper, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), of bridging the knowledge discrepancy between data and model. In TrustAL, our key idea is leveraging knowledge distillation~\cite{furlanello2018born}, which is orthogonally applicable to state-of-the-art AL methods~\cite{ash2019deep} focusing on data acquisition, in a synergistic manner.
Specifically, at each iteration, TrustAL searches for an expert predecessor model for the forgotten knowledge from a number of alternatives, then transfers the model knowledge (\eg, pseudo labels) to the current model training. By optimizing the dual goals of following not only oracle labels but also pseudo (soft) labels, the newly trained model can relieve example forgetting events, and thus be the trustworthy surrogate for the next data acquisition. For this purpose, we further explore the teacher selection problem: which predecessor is the most desired as a teacher for the forgotten knowledge? 

%Specifically, we present two teacher selection strategies: (i) monotonic choice of using the most recently trained model (\ie, a proxy of the most accurate model), and (ii) non-monotonic choice of using the well-balanced model with both accuracy and consistency. 


Our experiments show that TrustAL significantly improves performance with various data acquisition methods. We validate pseudo labels from the predecessor model are not just approximate/weak predictions \text{-} It can be viewed as knowledge from the previous generation, and can be used as consistency regularization for conventional AL methods solely aiming at higher accuracy.

==> backups/1_intro_before_review.tex <==
\section{Introduction} \label{sec:intro}

Labeling data is a fundamental bottleneck in machine learning due to annotation cost and time. One practical solution is Active Learning (AL): given a limited labeling budget $k$, which example should I ask human annotators to label?  Generally, this can be done through an \emph{iterative} process of data acquisition, labeling, and model training steps, until sufficient labels are obtained. At each iteration, based on the last trained model, unlabeled yet the $k$ most desirable examples are recognized and added to the labeled dataset to train a new model. This process continues to the next iteration for selecting next $k$ unlabeled examples based on the newly trained model. That is, a naive belief in AL is that the last trained model can be a good reference or surrogate for the distribution of the currently labeled data, which indicates what examples are desired for the next model update.


In this work, our empirical observation dispels this myth. Although the model knowledge learned from the labels is expected to be ``consistently'' kept or improved across AL iterations, we find that knowledge learned at some time is suddenly forgotten, which implies the ineligibility of the recent model to be treated as a good reference of the labeled dataset. More specifically, we can observe such inconsistent behaviors of the trained model during inference time, where sample $i$ predicted correctly at iteration $t$ is predicted incorrectly at iteration $t + \Delta t$, which is called \emph{example forgetting}~\cite{toneva2018empirical}. Here, we argue that prior AL methods only focusing on data acquisition steps~\cite{dasgupta2011two,xu2003representative,bodo2011active,ash2019deep} are still sub-optimal since such loss of knowledge deteriorates the quality of next data acquisition in an incremental manner during the whole AL generations. 


Motivated by this, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), of bridging the knowledge discrepancy between labeled data and model. In TrustAL, our key idea is to add a new step in the iterative process of AL to learn the forgotten knowledge, which is orthogonally applicable to state-of-the-art data acquisition strategies~\cite{ash2019deep} in a synergistic manner. Specifically, at each iteration, TrustAL first searches for a predecessor model from a number of alternatives as an expert model for the forgotten knowledge. Then, TrustAL transfers the model knowledge (\eg, logits) to the current model training step by leveraging the knowledge distillation techniques~\cite{hinton2015distilling}. By optimizing the dual goals of following not only human labels but also machine labels of the expert predecessor, the newly trained model can relieve example forgetting events, and thus be the trustworthy surrogate for the next data acquisition. 



For the purpose of identifying which predecessor is the most desired teacher for the forgotten knowledge, we further explore the teacher selection problem for better labeling. To resolve this, we present two teacher selection strategies, (1) \textbf{TrustAL-MC}: monotonic choice of the most recent model (\ie, a proxy of the most accurate model), 
and (2) \textbf{TrustAL-NC}: non-monotonic choice of the well-balanced model with accuracy and consistency, which we thoroughly design as analysis/evaluation measures in this paper. 


Our experiments show that the TrustAL framework significantly improves performance with various data acquisition strategies while preserving the valuable knowledge from the labeled dataset. We validate the pseudo labels from the predecessor models are not just approximate/weak predictions \text{-} It can be viewed as knowledge from the previous generation, and can be used as consistency regularization for conventional AL methods solely aiming at higher accuracy. 

==> backups/2_backup.tex <==



\subsection{Knowledge Distillation}
% Regularization based approach; incremental, L2 norm, ... and KD. We are different from using KD.
Knowledge distillation~\cite{hinton2015distilling} is designed to transfer knowledge from one model (the teacher model) to another (the student model) for compression of the large model. For that, knowledge distillation has been leveraged in learning that targeting in successive model generations. For example, in lifelong learning, knowledge distillation has been leveraged to compress the knowledge into the next generation model~\cite{ li2017learning, van2018generative}. Further, a number of recent papers~\cite{zhai2019lifelong, furlanello2018born, li2017learning} employ knowledge distillation for the purpose of minimizing forgetting in continual learning. In a similar vein, we employ knowledge distillation as a method for consistency regularization to address catastrophic forgetting for AL. 
% Specifically, while the teacher model is superior than the student model commonly in terms of accuracy, we use the inferior predecessor model as a teacher model to mitigate example forgetting.


% distill citatino 추가 
\subsection{Knowledge Distillation}\label{sec:pre.3}
Knowledge distillation~\cite{hinton2015distilling} is designed to transfer knowledge from one model (\ie, teacher model) to another (\ie, student model) for compression of the large model. 

lifelong learning~\cite{li2017learning,van2018generative,zhai2019lifelong,furlanello2018born,li2017learning} often leverages knowledge distillation to transfer the knowledge into the next generation model against catastrophic forgetting.

Unlike the typical use of knowledge distillation, we use the inferior predecessor model as a teacher model to mitigate example forgetting of the student model (\ie, last trained, superior model). Similarly, %, 

% 진영: 아주 짧은 한문장으로 차이점 말해주세요 .


%In a similar vein, we employ knowledge distillation as a method for consistency regularization to address catastrophic forgetting for AL. 




% 여기 accuracy가 왼쪽 축에서 오른쪽 축으로 오도록 서로 바꾸고, saturation event도 보이고, learning phase & forgetting phase 표시해야할까요? x 축 이름도 달라져야 할까요?

\begin{itemize}
    \setlength\itemsep{0.005em}
    \item \textbf{Stable phase:} Validation accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, where newly labeled samples improves generalization of the model being trained.
    \item \textbf{Saturated phase:} Validation accuracy converges or decreases with rapidly increasing MCI, suggesting that adding more data degrade the model generalization.
\end{itemize}

We present three main observation on accuracy and MCI dynamics based on the two phases we named above.\\
% #1 : Anti-correlated relationship (ACC - MCI)
\noindent\textbf{Observation 1} Across all dataset and acquisition strategies, accuracy and MCI follow the anti-correlated relationship in both phases. Accuracy tends to improve as the number of labeled dataset increases in the learning phase and MCI follows the reverse trend of accuracy. However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.\\
% #2 : anti correlated 된 상황에서 forgetting 줄이면 converge higher and faster 가능할 수도?
\noindent\textbf{Observation 2} We also observe the point of convergence in terms of accuracy is related to the convergence of MCI. Generally, we find the convergence of MCI is achieved earlier than accuracy while there exists minor deviation of the degree of the delay. 
% Controversial 한듯.. 어떻게 써야할까
We see this sequential convergence is a general phenomenon of AL and hypothesize that making more consistent model in the early stage may lead to higher accuracy with smaller labeling effort.\\
% #3 : label efficiency가 수렴한 이후에 떨어지는 현상이 일어남
\noindent\textbf{Observation 3} In addition, we find that after the convergence of accuracy, model starts to degrade, showing decreasing accuracy and exploding MCI. That is, the newly acquired labeled dataset after convergence period rapidly corrupts the generalization performance of model. One possible suspect might be outliers~\cite{karamcheti2021mind} which are samples that are mis- or ambiguously labeled, causing confusion of model. We further explore the effect of outliers in the Experiment section and show how our framework can successfully mitigate the adversarial effect of those samples.


==> backups/2_preliminary.tex <==

% issue list
% 1. lifelong learning 과 al의 차이점, 우리꺼에서 lifelong learning 기법을 어떤면에서 다르게 쓴거라고 볼수 있을까 해명(추후에 MC랑 엮어서 보여줘 버릴수도 있고)
% 2. https://www.ecva.net/papers/eccv_2020/papers_ECCV/papers/123710426.pdf al에 distill 쓴논문이 나왔네요
\section{Preliminaries \& Related Work} \label{sec:pre}


\subsection{Active Learning for Classification}\label{sec:pre.1}

Given an arbitrary classification task, assume that there is a large unlabeled dataset $\calU = \{x_i\}_{i=1}^n$ of $n$ data samples. The goal of AL is to sample a subset $\calQ \subset \calU$ to efficiently label so that newly training a deep neural network parameters $\theta$ for the classifier $f(x;\theta)$ improves test accuracy. Algorithm~\ref{alg:al} describes the conventional procedure in AL. On each iteration $t$, the learner uses strategy $\calA$ (\eg, uncertainty or diversity) to acquire $k$ samples $\calQ_t$ from dataset $\calU$. Generally, data acquisition model $M_t$ is used for evaluating unlabeled samples according to $\calA$. Then, for sample $x_i$, the learner queries for its oracle label $y_i \in 1,...,c$, where $c$ is the number of classes. We denote the predicted label of trained model $\theta_t$ for $x_i$ by $\hat{y}_i^t = argmax_{c} f(y_{ic}|x_i;\theta_t)$. %Note that, as our testbed, we focus on pool-based AL for text classification in this work.


    
\begin{algorithm}[h!]
\fontsize{9.5}{11.5}\selectfont
\STATE{\textbf{Input:} Initial labeled data pool $\calL$, unlabeled data pool $\calU$, number of queries per iteration (budget) $k$, number of iterations $T$, sampling algorithm $\calA$}\\
\STATE{\textbf{Output:} Model parameters $\theta_T$} \\
\STATE{$\theta_0 \leftarrow$ Train a seed model on $\calL$}\\
\For{iteration $t=1,...,T$}{
    \STATE{$M_t(x) = f(x;\theta_{t-1})$}\\
    \STATE{$\calQ_t$ $\leftarrow$ Apply $\calA(x, M_t, k)$ for $\forall x \in \calU$}\\
    \STATE{$\bar{\calQ}_t \leftarrow $ Label queries $\calQ_t$ by oracles}\\
    \STATE{$\calL \leftarrow \calL \cup \bar{\calQ}_t$}\\
    \STATE{$\calU \leftarrow \calU \setminus \bar{\calQ}_t$}\\
    \STATE{$\theta_t \leftarrow$ Train a new model on $\calL$}\\
}
\STATE{\textbf{return}~ $\theta_T$}
\caption{Conventional AL procedure}\label{alg:al}
\end{algorithm} 



In most AL approaches, a data acquisition model at time $t$ corresponds to the trained classification model at time $t\text{-}1$, \ie, $M_t = \theta_{t-1}$. We call this \textbf{monotonic acquisition}, since a naive belief would be assuming the last trained model $\theta_{t-1}$ is effective enough to not only provide a good representation for the entire labeled data $\calL$ but also estimate acquisition factors (\eg, confidence) for remaining unlabeled data $\calU$. 



\subsection{Data Acquisition Strategies in AL}\label{sec:pre.2}
The ultimate goal of AL is to improve the classification accuracy with a fixed annotation budget~\cite{settles2009active,lowell2018practical}. Existing research efforts on pool based active learning~\cite{lewis1994sequential} achieve this goal by focusing on data acquisition based on query strategy and data strategy~\cite{ren2020survey}. As a query strategy, there are two general approaches to recognize the most appropriate samples~\cite{dasgupta2011two} with monotonic acquisition: uncertainty sampling and diversity sampling. While uncertainty sampling efficiently searches the hypothesis space by finding difficult examples to label~\cite{asghar2017deep,he2019towards,ranganathan2017deep}, diversity sampling exploits heterogeneity in the feature space~\cite{hu2010off,bodo2011active}. Recently, hybrid approaches are proposed \cite{zhdanov2019diverse,ash2019deep}. Particularly, BADGE~\cite{ash2019deep} successfully integrates both aspects by clustering hallucinated gradient vectors based on monotonic acquisition scheme. 
% pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh pooh

% Meanwhile, data strategy can be orthogonally combined with assigning pseudo labels~\cite{wang2016cost,mittal2019parting}. In this paper, we propose to transfer the the knowledge from predecessor model for the purpose of restoring the lost knowledge utilizing logits as pseudo labels. 


\subsection{Data Acquisition Models in AL}\label{sec:pre.3}
Despite the remarkable success in query strategies, recent research has concerned several limitation of AL. \citet{yun2020weight,wang2016cost} point out the difficulty of learning good representation across AL iterations since insufficient annotations may lead to the instability of training models. This indicates that the monotonic acquisition does not ensure the last trained model as a good surrogate of the currently labeled data to identify the informative samples for data acquisition. As a result, \citet{karamcheti-etal-2021-mind,farquhar2020statistical,prabhu2019sampling} reveal that the acquired samples are vulnerable to sampling bias, and especially, \citet{karamcheti-etal-2021-mind} have presented Dataset Maps~\cite{swayamdipta2020dataset} of AL, which visualizes harmful outliers preferred by AL methods. Despite these facts, \citet{lowell2018practical} suggest that the monotonic acquisition is still promising as another remedy using external models (\eg, SVM out of the AL iterations) for data acquisition extremely hampers accuracy of AL.


Motivated by this line of research, in this work, we explore how the limitation of monotonic acquisition can be addressed, in particular, considering consistency as a solution to mitigate the instability of AL iterations. Similar to~\cite{lowell2018practical} reporting unreliable performance of AL in the NLP field, we choose text classification tasks as our testbed. 

% Data error detection also involves instance scor-
% ing. Influence functions (Koh and Liang, 2017),
% forgetting events (Toneva et al., 2018), cross valida-
% tion (Chen et al., 2019), Shapely values (Ghorbani
% and Zou, 2019), and the area-under-margin metric
% (Pleiss et al., 2020) have all been used to identify
% mislabeled examples. Some approaches avoid hard
% examples altogether (Bottou et al., 2005; Northcutt
% et al., 2017) to reduce fit to noisy data. Our use of
% training dynamics to locate mislabeled examples
% involves minimal additional effort beyond training
% a model on the dataset


% In this paper, we suggest a novel framework that conjugates data strategy using knowledge distillation and is orthogonally applicable to existing query strategies. 


==> backups/3_untrustworthy.tex <==

% \input{figure_files/figure-distributionbaseline}

% % random 제외한 버전
% \begin{figure*}[t!]\small
%     \begin{center}
%     \begin{tabular}{ccc}
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_conf_acc_ci_seeds.pdf, width=51mm} & 
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_coreset_acc_ci_seeds.pdf, width=51mm} &
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_badge_acc_ci_seeds.pdf, width=51mm} \\
%     (a) CONF & (b) CORESET & (c) BADGE \\
%     \end{tabular}
%     \end{center}
%     \caption{The distribution of example forgetting events; x-axis represents AL iterations and y-axis represents the mean correct inconsistency on left and the accuracy on right; (a) CONF, (b) CORESET, (c) BADGE}
%     \label{fig:exampleforgetting}
% \end{figure*}



\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_rand_acc_ci_seeds.pdf}
         \caption{Random sampling}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_conf_acc_ci_seeds.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_coreset_acc_ci_seeds.pdf}
         \caption{CORESET}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_trec_badge_acc_ci_seeds_ref_line_20.pdf}
         \caption{BADGE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_rand_acc_ci_seeds.pdf}
         \caption{Random sampling}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_conf_acc_ci_seeds.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_coreset_acc_ci_seeds.pdf}
         \caption{CORESET}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_badge_acc_ci_seeds_20.pdf}
         \caption{BADGE}
     \end{subfigure}
    % \caption{The accuracy and MCI on TREC (a\text{-}d) and on SST-2 (e\text{-}h) test data; x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics; We report the average values with five random seeds.}
    \caption{The accuracy and consistency (MCI) of Bi-LSTM model under three acquisition strategies on two text classification test datasets (TREC (a\text{-}d) and SST-2 (e\text{-}h)); x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics; We report the average values with five random seeds.}
    \label{fig:exampleforgetting}
\end{figure*}



\section{Accuracy-Consistency Dynamics}\label{sec:analysis.2}
In this section, we analyze the training dynamics of AL in terms of consistency along with accuracy, observing (catastrophic) \emph{example forgetting event}~\cite{toneva2018empirical} on the AL iterations: these occur when examples that have been ``learnt'' (\ie, correctly classified) at some time $t$ in the optimization process are subsequently misclassified -- or in other terms ``forgotten'' -- at a time $t\text{+}\Delta t > t$. Formally,

\newtheorem{definition}{Definition}
\begin{definition}{(Forgetting and Learning Events)}\label{def:forgetting}
Given a predicted label $\hat{y}_i^t$, let $\text{acc}_i^t = \mathbbm{1}_{\hat{y}^t_i = y_i}$ be a binary variable indicating whether the example is correctly classified by $\theta_t$. Sample $i$ undergoes a forgetting event when $acc_i^t$ decreases between two different iterations, \ie, $acc^{t}_i > acc^{t + \Delta t}_i$, where $\Delta t > 0$ (misclassified). Conversely, a learning event has occurred if $acc^{t}_i < acc^{t + \Delta t}_i$. 
\end{definition}


While learning new knowledge is also one of the important factors for generalization ability, our focus is on measuring how well models in AL preserve the learned knowledge. 
For further analysis, we introduce \textit{Correct Inconsistency} of a model as a measure of how inconsistent the target model is with its predecessor models for a sample. That is, correct inconsistency counts the forgetting events between the model and each of the predecessor models.

\begin{definition}{(Correct Inconsistency)}\label{def:ci}
The degree of correct inconsistency of $\theta_t$ for sample $x_i$ is measured as the number of occurrences of \textit{forgetting events} for sample $x_i$ from any predecessor model $\theta_{t-\Delta t}$, where $0 < \Delta t \leq t$:
\begin{equation*}
    \mathbb{C}^{(t)}_i = \sum_{\Delta t=1}^{t} \mathbbm{1}_{(acc^{t - \Delta t}_i > acc^{t}_i)}
\end{equation*}
\end{definition}


As the number of predecessor models are different per AL iteration, to fairly show the degree of inconsistency, we use mean of correct inconsistency for every sample in development split \eg, MCI =$ \sum_{i}{\mathbb{C}^{(t)}_i/t}$.

In Figure~\ref{fig:exampleforgetting}, we present both accuracy and MCI of trained models through the full progress of AL. We analyze three data acquisition strategies that are carefully chosen by considering the uncertainty-diversity dichotomy~\cite{yuan2020cold} along with random strategy. CONF~\cite{wang2014new}, CORESET~\cite{sener2017active}, and BADGE~\cite{ash2019deep} represent three lines of acquisition strategies in AL: uncertainty, diversity, and their hybrid. Across all dataset and acquisition strategies, accuracy and MCI follow the anti-correlated relationship. For convenience of analysis, we divide the training progress into two phases based on the transition of tendency in terms of accuracy: \emph{stable} and \emph{saturated} phases.


In the stable phase, more data leads to more accurate model. Validation accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, where newly labeled samples improve generalization of the trained models. In this phase, AL strategies seek to achieve label efficiency, reaching higher accuracy with a given amount of labeled samples or reversely achieving the same accuracy with less amount of labeled samples. What is notable here is that dramatic improvement of accuracy mostly involves the rapid drop in MCI. These analytical results provide a guide towards the idealistic property of AL methods, which is preserving existing knowledge and simultaneously learning new knowledge. Thus, we hypothesize that relieving forgetting events may contribute to faster and better (\ie, higher accuracy) convergence of AL.


In the saturated phase, the monotonic trends observed in stable phase do not hold. Validation accuracy converges or decreases with the rapid increase of MCI, suggesting that the generalization performance of model deteriorates as even more labeled samples are fed into the trained models. That is, more data does not always lead to more accurate model, which indicates labeling efforts may be negated in this phase. Although such an extremely undesirable situation in AL is barely addressed by stopping AL iterations in prior work~\cite{ishibashi2020stopping}, an idealistic AL framework would avoid this phase so that the models can be learned in a more label-efficient manner.


==> backups/3_untrustworthy_backup.tex <==
\section{Active Learning Might be Untrustworthy} \label{sec:analysis}


\subsection{Desired Characteristics for Active Learning} \label{sec:analysis.1}

\input{figure_files/figure-distributionbaseline}

We present two desired characteristics of trained model from the AL procedure.

An essential criterion for AL is that, as more data samples are consumed for training, the latter models have higher \textbf{accuracy} than the earlier models until the label efficiency (i.e. ratio of accuracy gain versus size of labeled set) converges. This is to ensure that as more data samples are learned, the model becomes more representative enough to identify informative samples among residual unlabeled dataset.

Existing research efforts aim to achieve this goal by focusing on data acquisition, especially with two general strategies~\cite{dasgupta2011two}: uncertainty sampling and diversity sampling. While uncertainty sampling efficiently searches the hypothesis space by finding difficult examples to label, diversity sampling exploits heterogeneity in the feature space~\cite{xu2003representative,hu2010off,bodo2011active}. Recently, BADGE~\cite{ash2019deep} successfully integrates both aspects by clustering confidence vectors. However, some lines of study reported unreliable performance of AL strategies across different dataset, model and .


Another practical criterion is \textbf{consistency}. \citet{wang2020wisdom} formally define \emph{consistency} of a model as the ability to make consistent predictions across successive model generations for the same input. There are several reasons to take such a criterion. One reason is that the consistency may determine the quality of monotonic data acquisition. The lack of consistency degrades trained models at each iteration and thus contaminates data acquisition in the next iterations. Such inefficiency causes redundant labeling costs. Another reason is that the consistency may determine the users' trust for model, which is of paramount importance. While software developers must repeat the similar test cases with redundant cost~\cite{spieker2019towards}, end users must deliberate when using the machine prediction for their decision making~\cite{ribeiro2016should}. 
However, compared to recent significant progress in terms of accuracy, consistency has not been explored enough in the AL field. 

Sampling bias is the most fundamental challenge posed by active learning. In this paper, we will deal exclusively with learning strategies that are provably consistent and we will analyze their label complexity: the number of labels queried in order to achieve a given rate of accuracy.~\cite{dasgusta2011two}

The main challenge in active learning is ensuring consistency~\cite{dasgupta2011two} in the agnostic setting while still maintaining low label complexity.
The loss of consistency is of practical concern as even popular active learning algorithms can induce inconsistency~\cite{dasgupta2011two}.

% 원래 두번째 
% Despite the discrepancies in terminology, almost every recent research on trustworthy AI agree on the need for building AI models that produce consistently correct outputs for the same input [14]. Although this seems like a straightforward requirement, however as we periodically retrain AI models in the field, there is no guarantee that different generations of the model will be consistently correct when presented with the same input.

\subsection{Accuracy-Consistency Dynamics}\label{sec:analysis.3}

To analyze the training dynamics of AL in terms of accuracy and consistency, we observe (catastrophic) \emph{example forgetting event}~\cite{toneva2018empirical} on the AL iterations: these occur when examples that have been ``learnt'' (\ie, correctly classified) at some time $t$ in the optimization process are subsequently misclassified -- or in other terms ``forgotten'' -- at a time $t\text{+}\Delta t > t$. Formally,

\newtheorem{definition}{Definition}%[section]
\begin{definition}{(Forgetting and Learning Events)}\label{def:forgetting}
Given a predicted label $\bar{y}_i^t$, let $\text{acc}_i^t = \mathbbm{1}_{\bar{y}^t_i = y_i}$ be a binary variable indicating whether the example is correctly classified by $\theta_t$. Sample $i$ undergoes a \emph{forgetting event} when $acc_i^t$ decreases between two different iterations, \ie, $acc^{t}_i > acc^{t + \Delta t}_i$, where $\Delta t > 0$ (misclassified). Conversely, a \emph{learning event} has occurred if $acc^{t}_i < acc^{t + \Delta t}_i$. 
\end{definition}

For further analysis, we introduce \textit{Correct Inconsistency} of a model as a measure of how inconsistent the target model is with predecessor models for a sample. That is, correct inconsistency counts the forgetting events between the model and each of the predecessor models.

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}%[section]
\begin{definition}{(Correct Inconsistency)}\label{def:ci}
The degree of (correct) inconsistency of $\theta_t$ is measured as the number of occurrences of \textit{forgetting events} for sample $x_i$ from any predecessor model $\theta_{t-\Delta t}$, where $0 < \Delta t < t$:
\begin{equation*}
    \mathbb{C}^{(t)}_i = \sum_{\Delta t=1}^{t-1} \mathbbm{1}_{(acc^{t - \Delta t}_i > acc^{t}_i)}
\end{equation*}
\end{definition}

% Beyond above sample-specific measures, we suggest an aggregated incosistency measure across all [seen] samples, namely mean correct inconsistency 
% \begin{equation*}
% MCI =\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}
% \end{equation*}

% Figure~\ref{fig:exampleforgetting} shows mean correct inconsistency (shortly, MCI $=\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}$), and accuracy of diverse acquisition strategies including uncertainty- and diversity-based samplings, CONF~\cite{wang2014new} and CORESET~\cite{sener2017active} respectively, and their hybrid sampling, BADGE~\cite{ash2019deep}, on TREC~\cite{roth2002question} and SST-2~\cite{socher2013recursive}. 

% In Figure~\ref{fig:exampleforgetting}, similar trends are commonly observed except for random sampling according to specific iterations, which we classify into the two:
% \begin{itemize}
%     \setlength\itemsep{0.005em}
%     \item \textbf{Stable learning:} Accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, which is the mainly focused iterations for AL scenarios. 
    
%     \item \textbf{Saturated learning:} After the first stage, accuracy almost converges, or decreases with dramatically increasing MCI.
% \end{itemize}

% Generally accuracy and MCI follow the anti-correlated relationship, perhaps because the forgotten status of the models affects the next data acquisition. 
% However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.

% Based on the above observation, by transferring the forgotten knowledge between AL cycles, relieving example forgetting events may contribute to higher accuracy. Here, correct inconsistency (Definition~\ref{def:ci}) can be re-used as a predictive metric to indicate the forgotten status of each model over all given samples (\eg, development set).

% accuracy of diverse acquisition strategies including uncertainty- and diversity-based samplings, CONF~\cite{wang2014new} and CORESET~\cite{sener2017active} respectively, and their hybrid sampling, BADGE~\cite{ash2019deep}, on TREC~\cite{roth2002question} and SST-2~\cite{socher2013recursive}. 

In Figure~\ref{fig:exampleforgetting}, we report the accuracy and mean correct inconsistency (MCI =$\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}$) of active learning. We observe a common patterns of active learner, albeit data increments toward maximum consumption: %[except for random sampling]: %  acquisition strategies including uncertainty- and diversity-based samplings

CONF~\cite{wang2014new} and CORESET~\cite{sener2017active} respectively, and their hybrid sampling, BADGE~\cite{ash2019deep}, on TREC~\cite{roth2002question} and SST-2~\cite{socher2013recursive}. 

\begin{itemize}
    \setlength\itemsep{0.005em}
    \item \textbf{Learning phase:} Accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases.  
    \item \textbf{Forgetting phase:} Accuracy almost converges, or decreases with dramatically increasing MCI, after the positive learning.
\end{itemize}

% Saturation variation
% which is the mainly focused iterations for AL scenarios.
We focus on the transition from the learning phase to the forgetting phase, and
Generally accuracy and MCI follow the anti-correlated relationship, perhaps because the forgotten status of the models affects the next data acquisition. 
However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.


Based on the above observation, by transferring the forgotten knowledge between AL cycles, relieving example forgetting events may contribute to higher accuracy. Here, correct inconsistency (Definition~\ref{def:ci}) can be re-used as a predictive metric to indicate the forgotten status of each model over all given samples (\eg, development set).


% 누락된 내용
% 1. knowledge about some data points is wasted, contradicting their goal for maximal data efficiency. 추가할지 논의 필요
% 2. 독자는 어려운 샘플과 쉬운 샘플이 있음을, 그리고 이것이 나중에 사용될 것을 짐작할 수 있어야할까. -> AL이 자꾸 forgetting하는 샘플을 고려하는 이유로 성능이 오른다는 분석을 주장하기 위해, 실험 4에서 sample-level importance에 따른 샘플의 차이를 대조하는 분석실험은 어떨까
% 3. \yeo{More details for the setting is presented in Appendix.}
% 4. (c)의 사진이 좀 더 불안정 (non-monotonic) 한 것으로 교체 필요



























==> backups/3_untrustworthy_before_review.tex <==
\section{Active Learning Might be Untrustworthy} \label{sec:analysis}

\input{figure_files/figure-distributionbaseline}



\subsection{Consistency in Active Learning}\label{sec:analysis.1}
Along with accuracy as a general criterion in AL, we argue that \textbf{correct-consistency} (which we call consistency for brevity) should be an essential criterion, which is the model ability to make consistent correct predictions across successive AL generations for the same input~\cite{wang2020wisdom}. In the practical point of view, consistency may determine the users' trust for model, which is of paramount importance. While developers must repeat the similar and redundant test cases without trust~\cite{spieker2019towards}, end users must deliberate when using the machine prediction for their decision making~\cite{ribeiro2016should}. 

To validate, we hypothesize that AL may suffer from inconsistency (reverse phenomenon of consistency), which we empirically analyze later in the experiment section.
\begin{itemize}
    \item \textbf{Sparse transition to model training:} Despite successful data acquisition, the subsequent labeling efforts can be negated by forgetting the learned knowledge later, which wastes annotation cost. We argue that consistency is key to make a label-efficient AL (Figure~\ref{fig:rq1-Trec}). 
    
    \item \textbf{Negative transition to data acquisition:} Inconsistent data acquisition models cannot serve as a good reference for the current data distribution, which leads to contaminating the next data acquisition step. Improving consistency may be synergetic to either uncertainty- or diversity-based acquisition strategies (Figure~\ref{fig:rq2}).
    
    \item \textbf{Careless transition from human labeling:} Human annotators act as oracles to provide infallible labels, but noisy labeling is one promising reason of example forgetting. Improving consistency enables learning to mitigate the confusion from the noisy labels (Figure 6).
\end{itemize}
However, consistency/inconsistency has not been explored enough in the AL field~\cite{dasgupta2011two}. 



\subsection{Accuracy-Consistency Dynamics}\label{sec:analysis.2}

We analyze the training dynamics of AL in terms of consistency along with accuracy, observing (catastrophic) \emph{example forgetting event}~\cite{toneva2018empirical} on the AL iterations: these occur when examples that have been ``learnt'' (\ie, correctly classified) at some time $t$ in the optimization process are subsequently misclassified -- or in other terms ``forgotten'' -- at a time $t\text{+}\Delta t > t$. Formally,

\newtheorem{definition}{Definition}
\begin{definition}{(Forgetting and Learning Events)}\label{def:forgetting}
Given a predicted label $\hat{y}_i^t$, let $\text{acc}_i^t = \mathbbm{1}_{\hat{y}^t_i = y_i}$ be a binary variable indicating whether the example is correctly classified by $\theta_t$. Sample $i$ undergoes a \emph{forgetting event} when $acc_i^t$ decreases between two different iterations, \ie, $acc^{t}_i > acc^{t + \Delta t}_i$, where $\Delta t > 0$ (misclassified). Conversely, a \emph{learning event} has occurred if $acc^{t}_i < acc^{t + \Delta t}_i$. 
\end{definition}
While learning new knowledge is also one of the important factors for generalization ability, our focus is on measuring how well models in AL preserves the learned knowledge. 
For further analysis, we introduce \textit{Correct Inconsistency} of a model as a measure of how inconsistent the target model is with predecessor models for a sample. That is, correct inconsistency counts the forgetting events between the model and each of the predecessor models.

\begin{definition}{(Correct Inconsistency)}\label{def:ci}
The degree of (correct) inconsistency of $\theta_t$ is measured as the number of occurrences of \textit{forgetting events} for sample $x_i$ from any predecessor model $\theta_{t-\Delta t}$, where $0 < \Delta t < t$:
\begin{equation*}
    \mathbb{C}^{(t)}_i = \sum_{\Delta t=1}^{t-1} \mathbbm{1}_{(acc^{t - \Delta t}_i > acc^{t}_i)}
\end{equation*}
\end{definition}


As the number of predecessor models are different per acquisition models, to fairly show the degree of inconsistency, we use mean of correct inconsistency for every sample in development split \eg, MCI =$\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}$.

In Figure~\ref{fig:exampleforgetting}, we present both accuracy and MCI of trained models through the full progress of AL. We analyze three data acquisition strategies that are carefully chosen by considering the uncertainty-diversity dichotomy~\cite{yuan2020cold} along with random strategy. CONF~\cite{wang2014new}, CORESET~\cite{sener2017active}, and BADGE~\cite{ash2019deep} represents three lines of strategy in AL: uncertainty, diversity, and their hybrid. Across all dataset and acquisition strategies, accuracy and MCI follow the anti-correlated relationship. For convenience of analysis in this section and the subsequent experiments, we divide the training progress into two phases based on the transition of tendency in terms of accuracy: Stable and saturated phases.


In the stable phase, more data leads to more accurate model. Validation accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, where newly labeled samples improve generalization of the trained models. In this phase, AL strategies seek to achieve label efficiency, reaching higher accuracy with a given amount of labeled samples or reversely achieving the same accuracy with less amount of labeled samples. What is notable here is that dramatic improvement of accuracy mostly involves the rapid drop in MCI. These analytical results provide a guide towards the idealistic property of AL methods, which is preserving existing knowledge and simultaneously learning new knowledge. Thus, we hypothesize that relieving forgetting events may contribute to faster and better (\ie, higher accuracy) convergence of AL.


In the saturated phase, the monotonic trends observed in stable phase does not hold. Validation accuracy converges or decreases with the rapid increase of MCI, suggesting that the generalization performance of model deteriorates as even more labeled samples are fed into the trained models. That is, not always more data leads to more accurate model, which indicates labeling efforts may be negated in this phase. Although such an extremely undesirable situation in AL is barely addressed by stopping AL iterations in prior work~\cite{ishibashi2020stopping}, an idealistic AL framework would avoid this phase so that the models can be learned in a more label-efficient manner.


==> backups/4_distillation.tex <==

\section{TrustAL: Trustworthy Active Learning}\label{sec:trustal}
Based on prior findings on training dynamics of AL procedure, we aim to relieve forgotten knowledge to train better acquisition model that serves as a good surrogate for labeled dataset. A naive way to obtain more generalized models is simply using enough labeled data. However, this approach is not always applicable since budget is limited in AL. Another line of work is using multiple equivalent models (\eg, ensemble) based on complementary nature across different generations. However, this approach is also not always affordable since querying on the huge pool of unlabeled data using multiple models is computationally too expensive.


We now present \textbf{TrustAL} (Trustworthy AL) that enables the training of consistent acquisition model that serves as a good reference for labeled dataset in smart and resource-efficient way. \textbf{TrustAL} utilizes additional machine generated labels for the purpose of mitigating the forgotten knowledge. Especially, among predecesor models, \textbf{TrustAL} identifies a proper expert model that can efficiently contribute to mitigating forgotten samples, which is a novel way of tackling the possible knowledge loss during AL procedure.




\subsection{Distillation-based Consistency Regularization}\label{sec:trustal.1}
Knowledge distillation~\cite{hinton2015distilling} is originally proposed to transfer knowledge from one model (\ie, teacher model) to another (\ie, student model) to compress the size of model. Inspired by recent approaches to transfer knowledge between equivalent models~\cite{furlanello2018born}, we propose using the inferior (\eg, less accurate) predecessor model as a teacher model to mitigate example forgetting of the student model (\ie, last trained, superior model) by learning from pseudo labels~(\ie{logits}). This distillation method can be interpreted as a type of consistency regularizer to alleviate forgotten knowledge.



% 여기 수식에 나오는 x, y 표기 좀 바꿔야 함 t가 의미하는 바랑 안맞음
Formally, Algorithm~\ref{alg:TrustAL} describes the overall procedure of the TrustAL framework on the AL iterations. When given a labeled data pool $\calL = \{x_i, y_i\}_{\forall i}$ at the $t$-th iteration, let $L_{CE}$ be a typical cross-entropy loss with oracle labeled examples, \ie, $\sum_{(x_i,y_i) \in \mathcal{L}} CrossEntropy(y_i, f(x_i;\theta_t))$,  and let $L_{KL}$ be a knowledge distillation loss with the pseudo labels of a predecessor model from $t\text{-}\Delta t$, \ie, $\sum_{(x_i,y_i) \in \mathcal{L}} KL\text{-}Divergence(f(x_i;\theta_{t-\Delta t}), f(x_i;\theta_t))$. On the top of an arbitrary data acquisition method (\eg, CORESET and BADGE), model parameter $\theta_t$ produced by TrustAL is obtained  by the following optimization:
\begin{equation} \label{eq:trustal}
    \theta_t = argmin_{\theta_t} L_{CE}(\theta_t) + \alpha \cdot L_{KL}( \theta_{t-\Delta t}, \theta_t)
\end{equation}
where $\alpha$ is a preference weight. We empirically analyze the effect of varying $\alpha$ in Appendix D. 


This framework motivates us to leverage more sophisticated techniques for knowledge distillation, such as~\cite{yuan2020revisiting,park2019relational}. We leave such exploration for future work, as using Eq. (\ref{eq:trustal}) works quite well for multiple AL methods in our experiments. 
Instead, as any predecessor model can be a teacher, we extend this framework to further exploration of teacher selection. 



\begin{algorithm}[t!]
    \fontsize{9.5}{11.5}\selectfont
    \caption{TrustAL}\label{alg:TrustAL}
    \STATE{\textbf{Input:} Initial labeled data pool $\calL_0$, unlabeled data pool $\calU$, number of queries per iteration (budget) $k$, number of iterations $T$, sampling algorithm $\calA$, fixed development dataset $\calD_{dev}$ with size $m$}\\
    \STATE{\textbf{Output:} Model parameters $\theta_T$}\\
    \STATE{$\theta_0 \leftarrow$ Train a seed model on \calL}\\
    \For{iteration $t=1,...,T$}{
        \STATE{$M_t(x) = f(x;\theta_{t-1})$}\\
        \STATE{$\calQ_t$ $\leftarrow$ Apply $\calA(x, M_t, k)$ for $\forall$ x $\in \calU$}\\
        \STATE{$\theta_{t-\Delta t} \leftarrow$ TeacherSelection$(\theta_0, ..., \theta_{t-1}, \calD_{dev})$}\\
        \STATE{$\bar{\calQ}_t \leftarrow $ Label queries $\calQ_t$ by oracles and $f(x;\theta_{t-\Delta t})$}\\
        \STATE{$\calL \leftarrow \calL \cup \bar{\calQ}_t$}\\
        \STATE{$\calU \leftarrow \calU\setminus \bar{\calQ}_t$}\\
        \STATE{$\theta_{t} \leftarrow$ $\operatorname*{argmin}_{\theta_t} L_{CE}(\theta_t) + \alpha \cdot L_{KL}(\theta_{t-\Delta t}, \theta_t)$}
    }

    \STATE{\textbf{return}~ $\theta_T$}
\end{algorithm}  


\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figure/process-diagram-0908-re.pdf}
\caption{Illustration of TrustAL-NC}
\label{fig:process-2}
\end{figure}

% \input{figure_files/figure-mainperformance}
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_conf_seeds_ens.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_coreset_seeds_ens.pdf}
         \caption{CORESET}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_badge_seeds_ens_ref_line.pdf}
         \caption{BADGE}
     \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_conf_seeds_ens.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_coreset_seeds_ens.pdf}
         \caption{CORESET}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_badge_seeds_ens.pdf}
         \caption{BADGE}
     \end{subfigure}
    \caption{Accuracy (a\text{-}c) and MCI (d\text{-}f) versus the ratio of labeled samples}
    % The results on the other dataset is in Appendix.}
    \label{fig:rq1-Trec}
\end{figure*}

\subsection{Teacher Selection Strategies}\label{sec:trustal.2}
The key factor of TrustAL framework is considering a predecessor model as a specialist model for the forgettable knowledge. As reported in Figure~\ref{fig:exampleforgetting}, specific to data increments across multiple generations, predecessor models have different status of learned and forgotten knowledge. Therefore, the distillation effects are different in how to select teacher models. Here, we introduce two strategies with TrustAL: monotonic and non-monotonic consistency.

\subsubsection{Monotonic Consistency (TrustAL-MC)}
Basically, we can inherit the monotonic approach not only for data acquisition but also for teacher selection, synchronizing both, \ie, always $\theta_{t-\Delta t} = \theta_{t-1} = M_t$. This allows to iteratively transfer the learned knowledge generation by generation. 



\subsubsection{Non-monotonic Consistency (TrustAL-NC)} \emph{Correct Inconsistency} (Definition~\ref{def:ci}) can be a strong signal to indicate which sample is forgettable for the current acquisition model. Using such sample level inconsistency, we aim at choosing the predecessor model with the learned knowledge especially of those forgettable samples. This allows to transfer the easily forgettable knowledge from one of the predecessor model, not always from $\theta_{t-\Delta t} = \theta_{t-1} = M_t$ as described in Figure~\ref{fig:process-2}. 





Specifically, given a development dataset $\calD_{dev}$ with $m$ samples, let $\mathbb{C}^{t}$ be a vector of correct inconsistency values of $M_t$ ($=\theta_{t-1}$) at the $t$-th iteration for all $m$ samples, \ie, $ \langle\mathbb{C}_1^{(t-1)},...,\mathbb{C}_m^{(t-1)}\rangle \in \mathbb{R}^{m}$. For the purpose of using this vector as importance weights for samples, we normalize $\mathbb{C}^{t}$ into $\Tilde{\mathbb{C}}^{t}$ where $\sum_{\forall i} \Tilde{\mathbb{C}}_i^{t} = 1$ by a softmax function. We note that the sample $x_i$ with high importance weight $\Tilde{\mathbb{C}}_i^{t}$ means easily forgettable sample for $M_t$. Based on such consistency-aware sample importance, we define a function $g(\theta_{t-\Delta t},M_t)$ of measuring how reliably a predecessor model $\theta_{t-\Delta t}$ can be a synergetic teacher with the data acquisition of $M_t$, by an weighted accuracy as:
\begin{equation}\label{eq:estimation}
    g(\theta_{t-\Delta t},M_t) = {\Tilde{\mathbb{C}}^{t}}{}^{\top} \langle acc_1^{t-\Delta t},...,acc_m^{t-\Delta t}\rangle / m
\end{equation}
High $g(\theta_{t-\Delta t},M_t)$ implies that the teacher model $\theta_{t-\Delta t}$ tends to have the knowledge of forgettable examples for the current data acquisition model $M_t$, and vice versa. Based on this, we can select a predecessor having the maximum value, as a teacher model to teach a new model $\theta_t$:
\begin{equation}\label{eq:estimation}
    \operatorname*{argmax}_{1 < \Delta t \leq t } g(\theta_{t-\Delta t},M_t)
\end{equation}
Note that the above estimation is a by-product of validation process without additional computations, which suggests that TrustAL is highly efficient compared to using ensemble-based approaches.








==> backups/5_experiments.tex <==
\section{Experiments}
\label{sec:experiment}

% issue list 
% distill 과 ensemble 성능 사이의 관계가 있다?
% acq - acq 는 여러가지 방법이 존재할 수 있지만 그 가능성을 보여주기 위해서 가장 naive한 방법론으로서 ensemble pseudo labeling을 제안하는 것이라고 설명하는게 좋을듯 ( 분명히 그냥 distill만 썻을때랑은 다른 모습을 보이기 때문에 의미는 있어 보이는데 powerful 한 method는 아직 우리가 못찾았기때문에 이렇게 주장하는 것이 덜 공격받고 후속 연구 활성화시키는데에 좋을듯)

\subsection{Experimental Setup}
\label{sec:experiment.1}

\subsubsection{Dataset} To validate the effectiveness of TrustAL, we use three text classification datasets, TREC~\cite{roth2002question}, Movie review~\cite{pang2005seeing} and SST-2~\cite{socher2013recursive}, which are widely used in AL~\cite{lowell2018practical,siddhant2018deep,yuan2020cold} and statistically diverse. 
The data statistics are presented in Appendix A for more details.


\subsubsection{Baselines} As TrustAL is orthogonally applicable to any data acquisition strategy, for the purpose of better analysis, we use the following three acquisition methods as baselines. 
\begin{itemize}
    \setlength\itemsep{0.0005em}
    \item \textbf{CONF}~\cite{wang2014new}: An uncertainty-based method that selects samples with least confidence.
    
    \item \textbf{CORESET}~\cite{sener2017active}: A diversity-based method that selects coreset of remaining samples. 
    
    \item \textbf{BADGE}~\cite{ash2019deep}: A hybrid method that selects samples considering both uncertainty and diversity.
\end{itemize}
More details on the baselines are discussed in Appendix B.


\subsubsection{Implementation}
For all three datasets, we follow the commonly used default settings in AL for text classification~\cite{liu2021deep,zhou2021towards,lowell2018practical,siddhant2018deep}: Bi-LSTM~\cite{hochreiter1997lstm} is adopted as a base model architecture; In each iteration of AL, training a classification model from scratch (not by incremental manner) with the entire labeled samples gathered, to avoid the training issues with warm-starting~\cite{ash2020warm}. We describe our implementation details in Appendix C.

% \input{figure_files/figure-heatmap}

\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[width=\textwidth]{figure/heatmap_trec_badge.pdf}
         \caption{TREC}
         \label{fig:sss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_mareview_badge.pdf}
         \caption{Movie Review}
     \end{subfigure}

     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_sst_badge.pdf}
         \caption{SST-2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_prev.pdf}
         \caption{Trust-MC on all dataset}
         \label{fig:sss}
     \end{subfigure}
    \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on three datasets with 5 random seeds. The $x$- and $y$-axis indicate the bins of the selected teacher model and the training model, respectively. In each round the size of labeled sample increases by 2\%. Each bin consists of 5 rounds. Brighter cell indicates more frequently selected bin.}
    \label{fig:heatmap}
\end{figure}

    % \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on (a) TREC, (b) Movie review and (c) SST-2. The $x$ and $y$ axes indicate the rounds of the selected teacher model and the rounds of the training model, respectively. Each round the labeled sample is increased by 2\%. The experiment is conducted with 5 random seeds for each round and is plotted in bins of 5 rounds. The brighter cell is, the more frequently selected rounds.}



\subsection{Results and Discussion}\label{sec:experiment.2}

We present the empirical findings for the following three research questions:

\noindent\textbf{RQ1: } Does TrustAL outperform AL baselines? 

\noindent\textbf{RQ2: } How does TrustAL help data acquisition?

\noindent\textbf{RQ3: } Does TrustAL make consistent and robust models?\\
Additional experiments on hyperparameter sensitivity are presented in Appendix D.
% \noindent\textbf{RQ4: } Is TrustAL insensitive to various factors?


\subsubsection{Overall Performance (RQ1)}\label{sec:new_rq_1}
First, we compare the performance of AL methods across AL iterations with and without TrustAL. Figure~\ref{fig:rq1-Trec} shows accuracy and MCI of AL methods on TREC. The empirical results in SST-2 and Movie Review are presented in Figure~\ref{fig:rq1-moviereview} and \ref{fig:ap.performance-sst} of Appendix F.

Overall, AL strategies combined with TrustAL-NC/MC show improved label efficiency and relieved MCI compared to stand-alone baselines in all datasets. The models trained with TrustAL framework require much smaller number of labeled samples to achieve the same level of accuracy than baselines. To facilitate the comparison of label efficiency of TrustAL and a baseline, we draw the horizontal reference line where the baseline starts to show convergence in Figure~\ref{fig:rq1-Trec} (c). As a result, we find that TrustAL-MC and TrustAL-NC require only 40\% and 30\% of the training data pool, respectively, while baselines requires 50\% of total training data to reach the same level of accuracy. This result suggests that keeping consistency of model in AL is an essential criterion, and TrustAL successfully satisfies the ultimate goal of AL, \ie, improving the label efficiency.

Further, TrustAL-NC performs comparably to ensemble\footnote{We use the implementation of~\cite{Fukuda2017EfficientKD}.} based distillation method. This indicates TrustAL-NC selects a teacher model that can effectively relieve forgotten knowledge, even without using all predecessor models. Figure~\ref{fig:heatmap} visualizes the behavior of teacher selection by TrustAL. The figure shows that TrustAL-MC selects the most recent model as its definition and TrustAL-NC chooses the teacher model based on the consistency guidance. While preferring the more generalized teacher models from the end of the stable learning stages (16-20) rather than earlier stages, TrustAL-NC also selects earlier generations that might be inferior but professional in terms of forgotten knowledge. That is, TrustAL-NC can select complementary models for forgotten knowledge in an automatic manner.


% Growing gap(Possible contents)
%For these results, a promising explanation is that this growing gap comes from the improvement of acquisition quality, triggering better model training and data acquisition in subsequent AL iterations. To validate this, we further analyze whether TrustAL actually improves acquisition quality in the data acquisition analysis section.


% \input{figure_files/figure-dataacquisition}
\begin{figure}[t!]\small
    \centering
     \begin{subfigure}[b]{0.38\textwidth}
         \includegraphics[width=\textwidth]{figure/data_acq_trec_conf_v2.pdf}
         \caption{CONF}
         \label{fig:conf}
     \end{subfigure}
     \hfill\\
     \begin{subfigure}[b]{0.38\textwidth}
         \includegraphics[width=\textwidth]{figure/data_acq_trec_coreset_v2.pdf}
         \caption{CORESET}
         \label{fig:div}
     \end{subfigure}
    \caption{Data acquisition analysis in stable phase on TREC; x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics.
    % The results on the other datasets are in Appendix.
    } \label{fig:rq2}
\end{figure}


% \input{figure_files/table-wangcc}
\begin{table}[t!]\small
\setlength\extrarowheight{3pt}
\centering
 \begin{tabular}{c l c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multicolumn{2}{c}{} & \textbf{TREC} & \textbf{Movie review}  & \textbf{SST-2} \\
\hline
\noalign{\hrule height0.8pt}
\multirow{4}{*}{A}    & baseline   & 0.726 & 0.637 & 0.686 \\\cline{2-5}
                         & Ensemble & 0.770 & 0.669 & 0.727 \\\cline{2-5}
                         & TrustAL-MC & 0.743 & 0.654 & 0.705 \\\cline{2-5}
                         & TrustAL-NC   & \textbf{0.774} & \textbf{0.676} & \textbf{0.730} \\\cline{1-5}
\multirow{4}{*}{B} & baseline & 0.727 & 0.627 & 0.697 \\\cline{2-5}
                         & Ensemble   & 0.777 & 0.658 & 0.724 \\\cline{2-5}
                         & TrustAL-MC & 0.753 & 0.654 & 0.707 \\\cline{2-5}
                         & TrustAL-NC   & \textbf{0.785} & \textbf{0.665} & \textbf{0.724} \\\cline{1-5}
\multirow{4}{*}{C}   & baseline   & 0.735 & 0.636 & 0.681 \\\cline{2-5}
                         & Ensemble   & 0.773 & 0.668 & 0.722 \\\cline{2-5}
                         & TrustAL-MC & 0.748 & 0.653 & 0.711 \\\cline{2-5}
                         & TrustAL-NC & \textbf{0.780} & \textbf{0.670} & \textbf{0.729} \\\cline{1-5}
 \hline
 \noalign{\hrule height0.8pt}
 \end{tabular}
\caption{Correct consistency of TrustAL-NC with (A) CONF (B) CORESET and (C) BADGE} 
\label{table:ap.wangcorrectconsistency}
\end{table}

\subsubsection{Data Acquisition Quality (RQ2)}\label{sec:new_rq_2} Having tested for the overall accuracy and MCI of TrustAL, we evaluate the quality of data acquisition results when using TrustAL. To discuss how TrustAL affects data acquisition, we analyze TrustAL-NC based on the two distinctive strategies on data acquisition: uncertainty and diversity. Note that, we choose to compare acquisition quality of stable phase only since the label efficiency of saturated phase is negative for traditional data acquisition strategies in AL.






For uncertainty, following~\cite{yuan2020cold}, we first obtain a reference model trained on the full training data of a target task, then measure the uncertainty of samples selected on each iteration. Specifically, by using Shannon Entropy~\cite{shannon2001mathematical}, we compute the entropy of the predicted probability distribution of individual samples, and report their average values for each AL iteration in Figure~\ref{fig:conf}, where a higher value implies each iteration successfully acquires uncertain samples.

For diversity, we reuse the reference model to encode the full training data into a feature space, then obtain the $k$ disjoint sets of the all training data by K-means algorithm where we set $k$ as the number of samples acquired per AL iterations. Then, based on these $k$ groups, we measure the diversity of a sample set selected on each iteration, by computing the entropy of a cluster distribution of the selected samples, which we report in Figure~\ref{fig:div}. The measure shows whether the samples are uniformly picked among the clusters, since diversely acquired samples would belong to different clusters~\cite{ash2019deep}. 


% 이거 그림 conf는 uncertainty만, coreset은 diversity만, badge는 둘다 그리는 걸로 바꾸는게 좋을듯

As shown in Figure~\ref{fig:rq2}, providing more labeled data leads to improvement of uncertainty and diversity for both baseline and TrustAL. Considering the reported increase of generalization performance in RQ1, this suggests that better model training leads to better acquisition, strengthening model's ability to identify more informative samples. For CONF and CORESET each representing uncertainty and diversity based strategies, we observe that TrustAL largely improves the quality of acquisition across the AL procedure. Since TrustAL aims to enhance the model's ability of surrogating the labeled dataset, we believe that TrustAL can be orthogonally and effectively applicable to any acquisition strategy with its synergetic nature.



\subsubsection{Model Consistency and Robustness (RQ3)}\label{sec:new_rq_3}

The correct consistency~\cite{wang2020wisdom}, $\ie, avg_{\forall i} \mathbbm{1}_{\hat{y}^m_i = \hat{y}^n_i = y_i}$, is a measure for the consistency between $m^{th}$ and $n^{th}$ generation models. By measuring the correct consistency between any two models, we demonstrate that our framework contributes not only to the label efficiency, but also to the overall consistency of model generations. Shown in Table~\ref{table:ap.wangcorrectconsistency}, TrustAL-NC shows better correct consistency than baselines. This reveals that models in AL iterations accord with each other for the correctly classified samples, which is also related to user's trust on system~\cite{wang2020wisdom}.
% since TrustAL-NC alleviates the example forgetting.



To demonstrate the robustness of TrustAL on the careless transition from human labeling, we deliberately corrupt the acquired samples by randomly flipping certain ratio of labels. Specifically, after stable phase, we corrupt 7\% and 15\% of the labels. In Figure~\ref{fig:noisy_label}, the result of BADGE and TrustAL(BADGE) are shown. Since other strategies show similar behaviors, we only present the result of BADGE. When the stable phase ends, the noisy labels cause the rapid increase of forgotten knowledge. Based on this observation, we believe that one of the possible suspect of performance degradation in the saturated phase might be noisy examples. Despite such degradation, TrustAL performs more robustly which is in strike contrast to the baseline. With 7\% of noise, TrustAL even shows comparable result to the one trained without noise. This result shows that TrustAL is robust to accidental noise in labels produced by human annotators since TrustAL regularizes the negative impact of such labels by pursuing consistency as an additional objective in training.







% Even after the generalization ability of model converges, AL strategies forces model to pick informative (\eg, least confident) samples. This causes the model to pick exotic samples that are hardly generalizable~\cite{karamcheti2021mind}. On the contrary to traditional AL framework, TrustAL naturally mitigates such adversarial impact of AL strategies by transferring knowledge from the predecessor so that AL framework can be more label efficient across the whole life cycle.

%\subsubsection{Parameter Sensitivity (RQ4)}\label{sec:new_rq_3}
%We present parameter sensitivity....  in Appendix for ...


% \input{figure_files/figure-noisylabel}
\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.22\textwidth}
         \includegraphics[width=\textwidth]{figure/noisy_label_0.07_acc.pdf}
        %  \caption{Noise ratio : 7\%}
         \label{fig:sss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.22\textwidth}
         
         \includegraphics[width=\textwidth]{figure/noisy_label_0.15_acc.pdf}
        %  \caption{Noise ratio : 15\%}
     \end{subfigure}

     \begin{subfigure}[t]{0.22\textwidth}
         
         \includegraphics[width=\textwidth]{figure/noisy_label_0.07_MCI.pdf}
         \caption{Noise ratio : 7\%}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.22\textwidth}
         \includegraphics[width=\textwidth]{figure/noisy_label_0.15_MCI.pdf}
         \caption{Noise ratio : 15\%}
         \label{fig:sss}
     \end{subfigure}
    \caption{Robustness analysis varying the ratio of noise. Accuracy and MCI are shown in pair for each noise ratio.}
    \label{fig:noisy_label}
\end{figure}

    % \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on (a) TREC, (b) Movie review and (c) SST-2. The $x$ and $y$ axes indicate the rounds of the selected teacher model and the rounds of the training model, respectively. Each round the labeled sample is increased by 2\%. The experiment is conducted with 5 random seeds for each round and is plotted in bins of 5 rounds. The brighter cell is, the more frequently selected rounds.}









==> backups/7_conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

% In this paper, we tackle the assumption in the conventional AL considering the consistency as a criterion for trustworthy model along with the accuracy. Based on observation, we propose TrustAL, a efficient algorithm which leverage knowledge distillation for maintaining consistency method. Further we suggest two strategies for TrustAL-MC which is based on monotonic consistency and TrustAL-NC with non-monotonic teacher selection. The extensive experiments demonstrate that our methods outperforms the baselines. Even TrustAL-NC shows the similar performance as ensemble model, which requires high cost. 

% Based on the empirical analysis using example forgetting,   in terms of inconsistency, we present a effective and robust framework, TrustAL, complementing the discrepancy which use knowledge distillation combined with any data acquisition strategies. As an extension, using teacher selection strategy, we suggest TrustAL-MC and TrustAL-NC, which improves accuracy and consistency significantly.

In this paper, we debunk the monotonicity assumption which is a common belief in conventional AL methods by empirical observation of example forgetting. For that, we present TrustAL, an effective and robust framework that uses the predecessor model as an expert model for knowledge distillation to compensate the loss of knowledge between data and model. Especially, our framework can be orthogonally applicable to existing data acquisition in a highly efficient way. Further, we present multi-pronged analysis for our method through extensive experiments. A promising future direction is to apply our approach to more complex and diverse tasks other than text classification task.




% text classification 이외의 task로 확대 적용하는 것

% task-balancing ability of TA between target task and pseudo-tasks, and make models broadly applicable to diverse NLP tasks.


%While existing AL methods mostly focus on the improvement of acquisition strategies to train better models, we argue that acquisition strategy and model are not independent in the process of AL, thus the label efficiency of a model does not solely rely on strategy. 

==> backups/backup_0829/1_backup_labeler.tex <==
\section{Introduction} \label{sec:intro}

% 구성
% 1. human label 이 ml에서 핵심 적인 요소이긴 하지만 cost가 너무 비쌈. 그래서 AL이 등장했고 최근에는 labeler를 accuracy와 cost가 다른 여러명으로 생각하고 푸는 work도 있다.

% 2. Motivated by diverse labeler scheme, 우리는 AL에서 학습 되는 machine을 하나의 additional labeler로서 활용하는 방법을 제안한다. Cost effective 하고, human labeler을 regularize하는 역할을 통해서 더 generalized 된 모델을 학습하는데에 도움을 준다고 hypothesize한다. label이 noisy한 경우(inconsistent or mislabeled)에도 machine labeler이 robust하게 성능을 유지하는데에 도움을 줄것이라고 생각한다.

% 3. Machine labeler가 labeler로서 AL에서 모델 학습 을 잘 도울 수 있는지를 알아보기 위해서(Proof of concept 차원에서) MC를 만들고 machine labeler를 쓰지 않았을 때와 비교해봤다. label-efficiency가 많이 개선되었다. 하지만 consistency가 그렇게 좋지 않아서, labeler로서 그냥 쓸수는 없음. Trust도 문제고 Inconsistent 한 label이 학습에 있어서 confusion을 발생시키기 때문임. human label 에서도 이런 일이 자주 일어나는데 그럴 때 성능이 매우 떨어지는 것을 확인할 수 있음. ex) movie review .. 그래서 이를 해결해야함.

% 4. MC의 발전된 버전을 만들기 위해서 우리는 NC를 제안한다. 이는 MC를 기준으로(Last model) inconsistency를 측정해서 그걸 지표로 삼아서 model을 골라 labeler 삼는 것이다. 이는 smart한 idea에서 비롯되는데 last model 이 labeled set의 어느정도의 surrogate으로 작동하기 때문에 MC가 잘맞추던 sample은 human label이 커버하게 되고 forget 된 샘플은 이전의 모델을 labeler로 삼음으로서 커버되기 때문이다. 이렇게 하면 MC 에서 inconsistent 했던 샘플들을 맞출 수 있도록 다음 모델이 학습되어서 consistent 해진다.

% 5. 실험을 통해서 봤더니, 매우 consistent 해졌고, labeling efficiency 가 굉장히 증가했음. 또한 매우 robust해져서 noisy label이 들어오는 상황에서도 망하지 않더라

% 글은 완전 미완성입니다.. 일단 생각 정리만 했습니다. (consensus가 먼저인거 같아서요)

Labeling data is a fundamental bottleneck in machine learning due to annotation cost and time. One practical solution is Active Learning (AL): given a limited labeling budget $k$, which example should I ask human annotators to label?  Generally, this can be done through an \emph{iterative} process of data acquisition, labeling, and model training steps, until sufficient labels are obtained. At each iteration, based on the last trained model, unlabeled yet the $k$ most desirable examples are recognized and added to the labeled dataset to train a new model. This process continues to the next iteration for selecting next $k$ unlabeled examples based on the newly trained model. That is, a naive belief in AL is that the last trained model can be a good reference or surrogate for the distribution of the currently labeled data, which indicates what examples are desired for the next model update.

While traditional AL framework assumes human annotator to be infallible, in many real settings, different labelers might have different annotation accuracies and show inconsistent because of underspecified or even missing guidelines, ambiguity, insufficient annotator expertise


This inconsistency of labels also . Especially for some tasks such as sentiment analysis, examples that is hard determine their labels are abundant. For example, ``XXXXXXXXXXXXXXXXXXXXX. " might be sorted as positive by some annotators while some would classify it as negative. Such inconsistent labeling is known to confuse the model causing significant failure in generalization ability. While annotating samples with soft labels are one of the powerful solutions, the cost of obtaining soft labels can be extremely huge.


in many real settings, different labelers might have different annotation costs and accuracies. That is, there exists strong labelers and weak labelers that demands higher and lower labeling cost each. Some recent works considered such setting \cite{zhang2015active,yan2016active} in AL and attempt to optimize the labeling efficiency using multiple annotators. \cite{gao2020cost} suggests an algorithm to select both labelers and instances to be labeled while assuming diverse labelers. 




Motivated by the approaches in diverse labelers setting, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), of using models produced during AL procedure as an additional oracle labeler for each step. In TrustAL, we consider last trained model, which is used for acquisition, as an additional annotator and so that provide additional labels for the samples gathered. However, naively utilizing the last trained model as an individual annotator may not be appropriate because of two reasons. 


The first reason is the inconsistency in labeling of machine annotators of each AL iterations. Although the model knowledge learned from the labels is expected to be ``consistently'' kept or improved across AL iterations, our empirical observation shows that knowledge learned at some time is suddenly forgotten. In other words, some correct predictions made by models are not kept after some steps of acquisition.












In this work, our empirical observation dispels this myth. Although the model knowledge learned from the labels is expected to be ``consistently'' kept or improved across AL iterations, we find that knowledge learned at some time is suddenly forgotten, which implies the ineligibility of the recent model to be treated as a good reference of the labeled dataset. More specifically, we can observe such inconsistent behaviors of the trained model during inference time, where sample $i$ predicted correctly at iteration $t$ is predicted incorrectly at iteration $t + \Delta t$, which is called \emph{example forgetting}~\cite{toneva2018empirical}. Here, we argue that prior AL methods only focusing on data acquisition steps~\cite{dasgupta2011two,xu2003representative,bodo2011active,ash2019deep} are still sub-optimal since such loss of knowledge deteriorates the quality of next data acquisition in an incremental manner during the whole AL generations. 


Motivated by this, we propose a label-efficient AL framework, called \textbf{Trust}worthy \textbf{AL} (\textbf{TrustAL}), of bridging the knowledge discrepancy between labeled data and model. In TrustAL, our key idea is to add a new step in the iterative process of AL to learn the forgotten knowledge, which is orthogonally applicable to state-of-the-art data acquisition strategies~\cite{ash2019deep} in a synergistic manner. Specifically, at each iteration, TrustAL first searches for a predecessor model from a number of alternatives as an expert model for the forgotten knowledge. Then, TrustAL transfers the model knowledge (\eg, logits) to the current model training step by leveraging the knowledge distillation techniques~\cite{hinton2015distilling}. By optimizing the dual goals of following not only human labels but also machine labels of the expert predecessor, the newly trained model can relieve example forgetting events, and thus be the trustworthy surrogate for the next data acquisition. 



For the purpose of identifying which predecessor is the most desired teacher for the forgotten knowledge, we further explore the teacher selection problem for better labeling. To resolve this, we present two teacher selection strategies, (1) \textbf{TrustAL-MC}: monotonic choice of the most recent model (\ie, a proxy of the most accurate model), 
and (2) \textbf{TrustAL-NC}: non-monotonic choice of the well-balanced model with accuracy and consistency, which we thoroughly design as analysis/evaluation measures in this paper. 


Our experiments show that the TrustAL framework significantly improves performance with various data acquisition strategies while preserving the valuable knowledge from the labeled dataset. We validate the pseudo labels from the predecessor models are not just approximate/weak predictions \text{-} It can be viewed as knowledge from the previous generation, and can be used as consistency regularization for conventional AL methods solely aiming at higher accuracy. 

==> backups/backup_0829/3_untrustworthy.tex <==
\section{Active Learning Might be Untrustworthy} \label{sec:analysis}


\subsection{Desired Characteristics for Active Learning} \label{sec:analysis.1}

\input{figure_files/figure-distributionbaseline}

We present two desired characteristics of trained model from the AL procedure. 

An essential criterion for AL is that, as more data samples are consumed for training, the latter models have higher \textbf{accuracy} than the earlier models. This is to ensure that as more data samples are learned, the model becomes more representative reference.
Existing research efforts achieve this characteristic by focusing on data acquisition, especially with two general strategies~\cite{dasgupta2011two}: uncertainty sampling and diversity sampling. While uncertainty sampling efficiently searches the hypothesis space by finding difficult examples to label, diversity sampling exploits heterogeneity in the feature space~\cite{xu2003representative,hu2010off,bodo2011active}. Recently, BADGE~\cite{ash2019deep} successfully integrates both aspects by clustering confidence vectors based on monotonic acquisition scheme.


%%%%% 젤 중요
% Another practical criterion is \textbf{correct-consistency} (which we call consistency for brevity). \citet{wang2020wisdom} formally define \emph{consistency} of a model as the ability to make consistent predictions across successive model generations for the same input. There are several reasons to take such a criterion. One reason is that inconsistency because of the sampling bias is the most fundamental challenge posed by active learning~\cite{dasgupta2011two}. Another reason is that there is no guarantee that different generations of the model will be consistently correct when presented with the same input~\cite{wang2020wisdom}. Further, the consistency may determine the quality of monotonic data acquisition. The lack of consistency degrades trained models at each iteration and thus contaminates data acquisition in the next iterations. Such inefficiency causes redundant labeling costs. 

%Such inefficiency causes wasting labeling costs
%Such vicious cycle of acquisition and training  causes redundant labeling costs in AL \cite{karamcheti2021mind}. 
% This paper studies a model
% behavior in the context of periodic retraining of deployed models where the outputs
% from successive generations of the models might not agree on the correct labels
% assigned to the same input

Another practical criterion is \textbf{correct-consistency} (which we call consistency for brevity). \citet{wang2020wisdom} formally define \emph{consistency} of a model as the ability to make consistent correct predictions across successive model generations for the same input. Consistency may determine the users' trust for model, which is of paramount importance. While software developers must repeat the similar and redundant test cases without trust~\cite{spieker2019towards}, end users must deliberate when using the machine prediction for their decision making~\cite{ribeiro2016should}. More technically, there are several reasons to take such a criterion. \yeo{One reason is that the trained model may negatively affect the next data acquisition not in a label-efficient manner. Due to the lack of consistency, the acquisition models cannot serve as a good reference for data distribution at each iteration, which thus contaminates data acquisition in the next iterations. We empirically analyze this in Figure~\ref{fig:rq1-Trec} later. Second, the data acquisition cannot be fully reflected on the model training to generalize the labeled knowledge. As forgetting the learned knowledge wastes the previous labeling efforts, the effect of uncertainty- or diversity-based sampling is degraded across iterations. We empirically analyze this in Figure 4 later. Finally, [[noise label, inconsistency label]]  } 
However, compared to recent significant progress in terms of accuracy, consistency has not been explored enough in the AL field~\cite{dasgupta2011two}. 



% Despite the discrepancies in terminology, almost every recent research on trustworthy AI agree on the need for building AI models that produce consistently correct outputs for the same input [14]. Although this seems like a straightforward requirement, however as we periodically retrain AI models in the field, there is no guarantee that different generations of the model will be consistently correct when presented with the same input.

\subsection{Accuracy-Consistency Dynamics}\label{sec:analysis.3}

To analyze the training dynamics of AL in terms of accuracy and consistency, we observe (catastrophic) \emph{example forgetting event}~\cite{toneva2018empirical} on the AL iterations: these occur when examples that have been ``learnt'' (\ie, correctly classified) at some time $t$ in the optimization process are subsequently misclassified -- or in other terms ``forgotten'' -- at a time $t\text{+}\Delta t > t$. Formally,

\newtheorem{definition}{Definition}%[section]
\begin{definition}{(Forgetting and Learning Events)}\label{def:forgetting}
Given a predicted label $\bar{y}_i^t$, let $\text{acc}_i^t = \mathbbm{1}_{\bar{y}^t_i = y_i}$ be a binary variable indicating whether the example is correctly classified by $\theta_t$. Sample $i$ undergoes a \emph{forgetting event} when $acc_i^t$ decreases between two different iterations, \ie, $acc^{t}_i > acc^{t + \Delta t}_i$, where $\Delta t > 0$ (misclassified). Conversely, a \emph{learning event} has occurred if $acc^{t}_i < acc^{t + \Delta t}_i$. 
\end{definition}

For further analysis, we introduce \textit{Correct Inconsistency} of a model as a measure of how inconsistent the target model is with predecessor models for a sample. That is, correct inconsistency counts the forgetting events between the model and each of the predecessor models.

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}%[section]
\begin{definition}{(Correct Inconsistency)}\label{def:ci}
The degree of (correct) inconsistency of $\theta_t$ is measured as the number of occurrences of \textit{forgetting events} for sample $x_i$ from any predecessor model $\theta_{t-\Delta t}$, where $0 < \Delta t < t$:
\begin{equation*}
    \mathbb{C}^{(t)}_i = \sum_{\Delta t=1}^{t-1} \mathbbm{1}_{(acc^{t - \Delta t}_i > acc^{t}_i)}
\end{equation*}
\end{definition}

% Figure~\ref{fig:exampleforgetting} shows mean correct inconsistency (shortly, MCI $=\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}$), and accuracy of diverse acquisition strategies including uncertainty- and diversity-based samplings, CONF~\cite{wang2014new} and CORESET~\cite{sener2017active} respectively, and their hybrid sampling, BADGE~\cite{ash2019deep}, on TREC~\cite{roth2002question} and SST-2~\cite{socher2013recursive}. 

% In Figure~\ref{fig:exampleforgetting}, similar trends are commonly observed except for random sampling according to specific iterations, which we classify into the two:
% \begin{itemize}
%     \setlength\itemsep{0.005em}
%     \item \textbf{Stable learning:} Accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, which is the mainly focused iterations for AL scenarios. 
    
%     \item \textbf{Saturated learning:} After the first stage, accuracy almost converges, or decreases with dramatically increasing MCI.
% \end{itemize}

% Generally accuracy and MCI follow the anti-correlated relationship, perhaps because the forgotten status of the models affects the next data acquisition. 
% However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.

Aggregating for every labeled samples as mean correct inconsistency, \eg, MCI =$\sum_{i}{\mathbb{C}^{(t)}_i/(t-1)}$, we monitor the learning curve during active learning on text classification task. In Figure~\ref{fig:exampleforgetting}, we plot both accuracy and MCI of trained learners under three data acquisition algorithms; CONF~\cite{wang2014new}, CORESET~\cite{sener2017active}, and  BADGE~\cite{ash2019deep}, as of each sampling is centered on uncertainty, diversity, and their hybrid, evaluated on dataset TREC~\cite{roth2002question} and SST-2~\cite{socher2013recursive}.

Considering random sampling as baseline, we observe two-phased patterns are common during AL's progress: % 여기 accuracy가 왼쪽 축에서 오른쪽 축으로 오도록 서로 바꾸고, saturation event도 보이고, learning phase & forgetting phase 표시해야할까요? x 축 이름도 달라져야 할까요?

\begin{itemize}
    \setlength\itemsep{0.005em}
    \item \textbf{Learning phase:} Accuracy increases on 0-50\% of TREC and 0-40\% of SST-2, while MCI decreases, which is the mainly focused scenario for AL.
    \item \textbf{Saturated phase:} Accuracy converges or decreases with rapidly increasing MCI, \ie the degree of forgetting outweighs that of learning.
\end{itemize}

Generally accuracy and MCI follow the anti-correlated relationship, perhaps because the forgotten status of the models affects the next data acquisition. 
As [AL uses an existing pool of labeled data as a proxy for the population of unlabeled examples]~\cite{kagy2019practical}, reducing the degree of forgetting may increase the model performance, which reaches higher accuracy in a shorter time or consumes more data in a prolonged learning phase. % Thus, we aim to decelerate the saturation of AL algorithms with counter-forgetting learners. In experiment #1, we show such learners prolong the learning phase of AL algorithms and, in result, learners themselves consume larger data volume.
However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.

Based on the above observation, by transferring the forgotten knowledge between AL cycles, relieving example forgetting events may contribute to higher accuracy and prolonged learning phase. Here, correct inconsistency (Definition~\ref{def:ci}) can be re-used as a predictive metric to indicate the forgotten status of each model over all given samples (\eg, development set).

% 누락된 내용
% 1. knowledge about some data points is wasted, contradicting their goal for maximal data efficiency. 추가할지 논의 필요
% 2. 독자는 어려운 샘플과 쉬운 샘플이 있음을, 그리고 이것이 나중에 사용될 것을 짐작할 수 있어야할까. -> AL이 자꾸 forgetting하는 샘플을 고려하는 이유로 성능이 오른다는 분석을 주장하기 위해, 실험 4에서 sample-level importance에 따른 샘플의 차이를 대조하는 분석실험은 어떨까
% 3. \yeo{More details for the setting is presented in Appendix.}
% 4. (c)의 사진이 좀 더 불안정 (non-monotonic) 한 것으로 교체 필요






% In learning phase, the accuracy and MCI follow the anti-correlated relationship, perhaps because the forgotten status of the models affects the next data acquisition. 
% As [AL uses an existing pool of labeled data as a proxy for the population of unlabeled examples]~\cite{kagy2019practical}, reducing the degree of forgetting may increase the model performance, which reaches higher accuracy in a shorter time or consumes more data in a prolonged learning phase. % Thus, we aim to decelerate the saturation of AL algorithms with counter-forgetting learners. In experiment #1, we show such learners prolong the learning phase of AL algorithms and, in result, learners themselves consume larger data volume.
% However, while accuracy shows roughly monotonic patterns, MCI is not the case with fluctuating values across AL iterations. This suggests that the conventional monotonic acquisition merely depending on the last trained model is sub-optimal in terms of MCI although it looks near-optimal in terms of accuracy.

% Based on the above observation, by transferring the forgotten knowledge between AL cycles, relieving example forgetting events may contribute to higher accuracy and prolonged learning phase. Here, correct inconsistency (Definition~\ref{def:ci}) can be re-used as a predictive metric to indicate the forgotten status of each model over all given samples (\eg, development set).





















==> backups/backup_0829/6_related.tex <==
\section{Related Work}

\noindent\textbf{Model Consistency}
Although catastrophic forgetting events occur inevitably~\cite{toneva2018empirical} in continual learning, there are only a limited number of studies related to consistency. While \citet{anil2018large} propose a distillation method for reproducing the same predictions without focusing on measuring the consistency, \citet{wang2020wisdom} define consistency and correct-consistency of a model and propose ensemble methods for consistency. Inspired by this, we suggest correct-inconsistency of a model as a measure for estimating the knowledge loss and use it as a guidance in our method.


% \vspace{2mm}
% \noindent\textbf{Knowledge Distillation} Knowledge distillation has been used in lifelong learning ~\cite{lifelongnlp-2020-life, li2017learning, van2018generative} to compress the knowledge into the next generation model. Meanwhile, we leverage knowledge distillation as method for a consistency regularizer to maintaining the consistency, which also yields improvement in terms of the accuracy.

\vspace{2mm}
\noindent\textbf{Data Acquisition for Active Learning} To achieve better performance in AL, existing work focuses on the data acquisition step using query strategy and data strategy~\cite{ren2020survey}. As a query strategy, there are uncertainty-based~\cite{beluch2018power, ranganathan2017deep, wang2014new}, diversity-based~\cite{sener2017active, gal2017deep} and hybrid approaches~\cite{ash2019deep, shui2020deep} with monotonic acquisition. Meanwhile, data strategy is possible such as assigning pseudo-label~\cite{wang2016cost} and data augmentation using GAN~\cite{tran2019bayesian, zhu2017generative}. In this paper, we analyze each strategy and suggest a novel framework that conjugates data strategy using knowledge distillation and is combined with query strategy in an orthogonal manner. 

%Meanwhile, we leverage knowledge distillation as a method for consistency regularization, which yields improvements on both accuracy and consistency.






% issues
% 1) continual learning이 완전히 우리의 세팅은 아님. 이에 대한 부가적인 설명 필요.
% 2) continual learning에 CF 내용이 들어가는데, example forgetting을 CF의 일부로 보는 논문들이 존재함. discuss 필요.
% 3) example forgetting 필요시 https://arxiv.org/pdf/1812.05159.pdf 의 수식 추가
% 4) knowledge distillation 파트에 continual에서 distill을 쓴 것 & 작은 모델에서 큰 모델로의 distill에 대한 강조 를 추가하고 싶음.

% \section{Related Work}
% \subsection{Continual Learning} % dumped from https://arxiv.org/pdf/2012.09823.pdf /// https://arxiv.org/pdf/1805.12369.pdf /// https://ojs.aaai.org/index.php/AAAI/article/view/7079/6933
% Continual learning(CL) is a machine learning paradigm, whose objective is to adaptively learn across time by leveraging previously learned tasks to improve generalization for future tasks. Hence, CL studies the problem of sequential learning from a continuous stream of data, drawn from a potentially non-stationary distribution, and reusing gained knowledge throughout the lifetime while avoiding catastrophic forgetting(CF). CF means that when a neural network learns a sequence of tasks, the learning of each new task is likely to change the weights learned for previous tasks, which degrades the model accuracy for the previous tasks (McCloskey and Cohen, 1989). 

% % dumped from https://arxiv.org/pdf/1903.12648.pdf

% The primary goal of CL is to overcome the forgetting of learned tasks and to leverage the earlier knowledge for obtaining better performance or faster convergence/training speed on the newly coming tasks.



% % possibly skipped
% \subsection{Example Forgetting}
% % dumped from https://arxiv.org/pdf/1911.03861.pdf
% An example is forgotten if it goes from being correctly to incorrectly classified during training (each such occurrence is called a forgetting event). This happens due to the stochastic nature of gradient descent, in which gradient updates performed on certain examples can hurt performance on others. If an example is forgotten at least once or is never learned during training it is dubbed forgettable. Finding forgettable examples entails training the model on $\mathcal{D}$ and tracking the accuracy of each example at each presentation during training. The algorithm for computing forgettability is cheap (Toneva et al., 2019) and only requires storing the accuracy of each particular example at each epoch.

\subsection{Knowledge Distillation}
% dumped from https://arxiv.org/pdf/1805.04770.pdf 
% https://openaccess.thecvf.com/content_ICCV_2019/papers/Hou_Learning_Lightweight_Lane_Detection_CNNs_by_Self_Attention_Distillation_ICCV_2019_paper.pdf
% https://openaccess.thecvf.com/content_CVPR_2019/papers/Park_Relational_Knowledge_Distillation_CVPR_2019_paper.pdf
There has been a long line of research and development on transferring knowledge from one model to another. Sometimes the goal is compression: to produce a compact model that retains the accuracy of a larger model that takes up more space and/or requires more computation to make predictions (Bucilua et al., 2006; Hinton et al., 2015). Breiman and Shang [3] first proposed to learn singletree models that approximate the performance of multipletree models and provide better interpretability. Similar approaches for neural networks have been emerged in the work of Bucilua et al. [4], Ba and Caruana [1], and Hinton et al. [11], mainly for the purpose of model compression. Bucilua et al. compress an ensemble of neural networks into a single neural network. Ba and Caruana [1] increase the accuracy of a shallow neural network by training it to mimic a deep neural network with penalizing the difference of logits between the two networks. Hinton et al. [11] revive this idea under the name of KD that trains a student model with the objective of matching the softmax distribution of a teacher model.

A few recent papers [2, 9, 45] have shown that distilling a teacher model into a student model of identical architecture, i.e., self-distillation, can improve the student over the teacher. Furlanello et al. [9] and Bagherinezhad et al. [2] demonstrate it by training the student using softmax outputs of the teacher as ground truth over generations. Yim et al. [45] transfers output activations using Gramian matrices and then fine-tune the student.

Also, interest in KD has also spread beyond supervised learning. A number of recent papers (Furlanello et al., 2016; Li & Hoiem, 2016; Shin et al., 2017) employ KD for the purpose of minimizing forgetting in continual learning.









==> backups/hongin.tex <==
% 홍인
% work in progress...

% writing 아이디어 1
% 주제: saturation AL -> economic interaction among a lineage of active learners
% consumer : active learner
% producer: consumer in past (backbone network that serves as "engine" of data acquisition algorithms)
% what consumer want: collect knowledge at each round
% what producer want: sell data that is most uncertain & diver to their knowledge 
% product: a batch of labeled data (consumer - "examples" -> producer)
% currency: customer (which have some knowledge) pay the cost of re-parameterization
% good purchase: consumer's knowledge increase (successful learning from data batch)
% bad purchase: consumer's knowledge decrease or converge (bad learning from data batch)
% knowledge affordability in general: model capacity
% knowledge affordability in AL: "data acquisition quality" + model capacity
% saturation in AL: more unlabeled data available, but no consumer gain knowledge from it

% writing 아이디어 2
% 주제: monotone vs non-monotone -> example-confusion 과 knowledge-of-memory 비유
% why do producer fail in AL: because the producer don't sell what consumer want and need
% what should producer do: producer must reconsider its own knowledge (that control the data acquisition)
% how should producer do: producer must consider the need of customer -> what kind of examples did previous customers needed extra help?
% what does correct-inconsistency mean: statistics of customer needs (just like market analysis or customer report)
% what is sample importance C: an example-confusion report as customer feedback. This report is created by a direct survey on a group of previous customers that counts on which examples they keep forgetting and learning back and forth.
% what is selection score g: a confusion-weighted accuracy; the performance of each model that weigh accuracy in favor of countering example-confusion; higher the confusing the examples are, higher we value the accuracy of a correct prediction
% what is selected model theta: an expert specialized on the confusing examples in AL; it got the confusing examples most correctly where examples were kept learned and forgotten though the AL cylces
% what would the selected model do: 1) select unlabeled data as a knowledge-without-confusion expert, examined on labeled data in their memory 2) regularize the consumer to learn their knowledge-without-confusion by standardizing their consistent prediction
% why knowledge distillation: transfer knowledge-without-confusion to consumer -> better than ensemble because they transfer knowledge-with-confusion also 
% why do we consider feedback from the global past: ? local past ...

% Goal: TrustAL-NC propose a example-level predictive consistency in AL cycle.
% Challenge: 1) example-confusion 2) forgotten knowledge
% Solution: enforce traditional AL algorithms 1) consistent behavior of active learners 2) transfer forgotten knowledge across generation 
% Method: 1) select data based on "model with minimal confusion" 2) actively learn from "model with minimal confusion"


==> backups/macros.tex <==
\newtheorem{example}{Example}

\newcommand\Tstrut{\rule{0pt}{2.2ex}}       % "top" strut
\newcommand\Bstrut{\rule[-0.6ex]{0pt}{0pt}} % "bottom" strut
\newcommand{\TBstrut}{\Tstrut\Bstrut} % top&bottom struts

\newcommand{\se}{{\it SE}}%
\newcommand{\eg}{{\it e.g.}}%
\newcommand{\ie}{{\it i.e.}}%
\newcommand{\etal}{{\it et al.}}%
\newcommand{\etc}{{\it etc}}%
\newcommand{\ours}{{ALT-TAB}}%
\newcommand{\kmeans}{\text{k-MEANS++}}%


%  colors
\newcommand{\todoc}[2]{{\textcolor{#1}{{#2}}}}
\newcommand{\todoblue}[1]{\todoc{blue}{{#1}}}
% \definecolor{pgreen}{rgb}{0.13, 0.40, 0.23} 
% \definecolor{ppurple}{rgb}{0.39, 0.37, 0.76}
% \newcommand{\todoorange}[1]{\todoc{pgreen}{{#1}}}
\newcommand{\hong}[1]{\todoc{purple}{#1}} % 홍인
 \newcommand{\yeo}[1]{\todoblue{#1}} % 진영
\newcommand{\pooh}[1]{\todoorange{#1}} % 유진
% \newcommand{\bwoo}[1]{\todoc{pgreen}{#1}} % 병우
\newcommand{\swTodo}[1]{\todored{#1}}

% Caligraphy style
\newcommand{\mcal}[1]{{\cal{#1}}}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calB}{\mbox{${\cal B}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calE}{\mbox{${\cal E}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calG}{\mbox{${\cal G}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\calJ}{\mbox{${\cal J}$}}
\newcommand{\calK}{\mbox{${\cal K}$}}
\newcommand{\calL}{\mbox{${\cal L}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calN}{\mbox{${\cal N}$}}
\newcommand{\calO}{\mbox{${\cal O}$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calQ}{\mbox{${\cal Q}$}}
\newcommand{\calR}{\mbox{${\cal R}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calU}{\mbox{${\cal U}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calW}{\mbox{${\cal W}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}
\newcommand{\calZ}{\mbox{${\cal Z}$}}

\newcommand*\concat{\mathbin{\|}}

==> figure_files/figure-dataacquisition.tex <==
\begin{figure}[t!]\small
    \centering
     \begin{subfigure}[b]{0.38\textwidth}
         \includegraphics[width=\textwidth]{figure/data_acq_trec_conf_v2.pdf}
         \caption{CONF}
         \label{fig:conf}
     \end{subfigure}
     \hfill\\
     \begin{subfigure}[b]{0.38\textwidth}
         \includegraphics[width=\textwidth]{figure/data_acq_trec_coreset_v2.pdf}
         \caption{CORESET}
         \label{fig:div}
     \end{subfigure}
    \caption{Data acquisition analysis in stable phase on TREC; x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics.
    % The results on the other datasets are in Appendix.
    } \label{fig:rq2}
\end{figure}


==> figure_files/figure-distributionbaseline.tex <==

% % random 제외한 버전
% \begin{figure*}[t!]\small
%     \begin{center}
%     \begin{tabular}{ccc}
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_conf_acc_ci_seeds.pdf, width=51mm} & 
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_coreset_acc_ci_seeds.pdf, width=51mm} &
%     \epsfig{file=acl-ijcnlp2021-templates/figure/figure1_badge_acc_ci_seeds.pdf, width=51mm} \\
%     (a) CONF & (b) CORESET & (c) BADGE \\
%     \end{tabular}
%     \end{center}
%     \caption{The distribution of example forgetting events; x-axis represents AL iterations and y-axis represents the mean correct inconsistency on left and the accuracy on right; (a) CONF, (b) CORESET, (c) BADGE}
%     \label{fig:exampleforgetting}
% \end{figure*}



\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_rand_acc_ci_seeds.pdf}
         \caption{Random sampling}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_conf_acc_ci_seeds.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_coreset_acc_ci_seeds.pdf}
         \caption{CORESET}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_trec_badge_acc_ci_seeds_ref_line_20.pdf}
         \caption{BADGE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_rand_acc_ci_seeds.pdf}
         \caption{Random sampling}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_conf_acc_ci_seeds.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_coreset_acc_ci_seeds.pdf}
         \caption{CORESET}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure1_sst2_badge_acc_ci_seeds_20.pdf}
         \caption{BADGE}
     \end{subfigure}
    % \caption{The accuracy and MCI on TREC (a\text{-}d) and on SST-2 (e\text{-}h) test data; x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics; We report the average values with five random seeds.}
    \caption{The accuracy and consistency (MCI) of Bi-LSTM model under three acquisition strategies on two text classification test datasets (TREC (a\text{-}d) and SST-2 (e\text{-}h)); x-axis represents the ratio of labeled samples and y-axis represents the corresponding metrics; We report the average values with five random seeds.}
    \label{fig:exampleforgetting}
\end{figure*}



==> figure_files/figure-heatmap.tex <==
\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[width=\textwidth]{figure/heatmap_trec_badge.pdf}
         \caption{TREC}
         \label{fig:sss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_mareview_badge.pdf}
         \caption{Movie Review}
     \end{subfigure}

     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_sst_badge.pdf}
         \caption{SST-2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\textwidth}
         
         \includegraphics[width=\textwidth]{figure/heatmap_prev.pdf}
         \caption{Trust-MC on all dataset}
         \label{fig:sss}
     \end{subfigure}
    \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on three datasets with 5 random seeds. The $x$- and $y$-axis indicate the bins of the selected teacher model and the training model, respectively. In each round the size of labeled sample increases by 2\%. Each bin consists of 5 rounds. Brighter cell indicates more frequently selected bin.}
    \label{fig:heatmap}
\end{figure}

    % \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on (a) TREC, (b) Movie review and (c) SST-2. The $x$ and $y$ axes indicate the rounds of the selected teacher model and the rounds of the training model, respectively. Each round the labeled sample is increased by 2\%. The experiment is conducted with 5 random seeds for each round and is plotted in bins of 5 rounds. The brighter cell is, the more frequently selected rounds.}

==> figure_files/figure-mainperformance.tex <==
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_conf_seeds_ens.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_coreset_seeds_ens.pdf}
         \caption{CORESET}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_acc_badge_seeds_ens_ref_line.pdf}
         \caption{BADGE}
     \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_conf_seeds_ens.pdf}
         \caption{CONF}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_coreset_seeds_ens.pdf}
         \caption{CORESET}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/figure3_trec_ci_badge_seeds_ens.pdf}
         \caption{BADGE}
     \end{subfigure}
    \caption{Accuracy (a\text{-}c) and MCI (d\text{-}f) versus the ratio of labeled samples}
    % The results on the other dataset is in Appendix.}
    \label{fig:rq1-Trec}
\end{figure*}

==> figure_files/figure-noisylabel.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.22\textwidth}
         \includegraphics[width=\textwidth]{figure/noisy_label_0.07_acc.pdf}
        %  \caption{Noise ratio : 7\%}
         \label{fig:sss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.22\textwidth}
         
         \includegraphics[width=\textwidth]{figure/noisy_label_0.15_acc.pdf}
        %  \caption{Noise ratio : 15\%}
     \end{subfigure}

     \begin{subfigure}[t]{0.22\textwidth}
         
         \includegraphics[width=\textwidth]{figure/noisy_label_0.07_MCI.pdf}
         \caption{Noise ratio : 7\%}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.22\textwidth}
         \includegraphics[width=\textwidth]{figure/noisy_label_0.15_MCI.pdf}
         \caption{Noise ratio : 15\%}
         \label{fig:sss}
     \end{subfigure}
    \caption{Robustness analysis varying the ratio of noise. Accuracy and MCI are shown in pair for each noise ratio.}
    \label{fig:noisy_label}
\end{figure}

    % \caption{Heatmap showing frequency of the model selection in TrustAL-NC with BADGE on (a) TREC, (b) Movie review and (c) SST-2. The $x$ and $y$ axes indicate the rounds of the selected teacher model and the rounds of the training model, respectively. Each round the labeled sample is increased by 2\%. The experiment is conducted with 5 random seeds for each round and is plotted in bins of 5 rounds. The brighter cell is, the more frequently selected rounds.}

==> figure_files/table-sensitivity-MC.tex <==
\begin{table*}[t]\small
\setlength\extrarowheight{3pt}
\centering
 \begin{tabular}{c c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{} & &\multicolumn{2}{c}{\textbf{Stable Learning Stage}} &\multicolumn{2}{c}{\textbf{Saturated Learning Stage}}\\\cline{3-6}
                   & &\textbf{accuracy} & \textbf{MCI} & \textbf{accuracy} & \textbf{MCI} \\
\hline
\noalign{\hrule height0.8pt}
\multirow{5}{*}{KD Loss Hyp.} & 0.3 & 0.774(\textcolor{pgreen}{-0.004}) & 24.82(\textcolor{pgreen}{+3.07}) & 0.855(\textcolor{pgreen}{0.007}) & 22.40(\textcolor{pgreen}{-3.17}) \\\cline{2-6}
                              & 0.75* & 0.779(\textcolor{pgreen}{+0.001}) & 23.68(\textcolor{pgreen}{+1.93}) & 0.862(\textcolor{pgreen}{+0.014}) & 20.02(\textcolor{pgreen}{-5.55}) \\\cline{2-6}
                              & 1.5 & 0.787(\textcolor{pgreen}{+0.008}) & 18.84(\textcolor{pgreen}{-2.90}) & 0.874(\textcolor{pgreen}{+0.026}) & 21.27(\textcolor{pgreen}{-4.30}) \\\cline{2-6}
                              & 10 & 0.818(\textcolor{pgreen}{+0.040}) & 16.01(\textcolor{pgreen}{-5.74}) & 0.871(\textcolor{pgreen}{+0.023}) & 22.27(\textcolor{pgreen}{-3.29}) \\\cline{2-6}
                              & 20 & 0.789(\textcolor{pgreen}{+0.011}) & 15.84(\textcolor{pgreen}{-5.91}) & 0.878(\textcolor{pgreen}{+0.030}) & 13.26(\textcolor{pgreen}{-12.31}) \\\cline{1-6}
 \hline
 \noalign{\hrule height0.8pt}
 \end{tabular}
\caption{Performance of TrustAL-MC with BADGE on TREC for sensitivity analysis. The colored numbers are the difference between BADGE with each hyper-parameter (green: improvement, purple: deterioration). The performance is the average performance of each phase. The hyper-parameter of the experiment on section ~\ref{sec:new_rq_1} are marked with *. The results with the other AL algorithms are in Appendix.} 
\label{table:sensitivity-MC}
\end{table*}

==> figure_files/table-sensitivity-bert.tex <==
\begin{table}[h]\small
\setlength\extrarowheight{3pt}
\centering
 \begin{tabular}{c l c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{} & &\multicolumn{2}{c}{\textbf{Stable}} &\multicolumn{2}{c}{\textbf{Saturated}}\\\cline{3-6}
  \multirow{2}{*}{} & &\textbf{acc.} & \textbf{MCI}  & \textbf{acc.} & \textbf{MCI}\\
\hline
\noalign{\hrule height0.8pt}
\multirow{2}{*}{A}    & baseline  & 0.759  & 159.6 & 0.844 & 70.0 \\\cline{2-6}
                         & TrustAL-NC  & 0.764  & 154.7  & 0.848 & 65.6 \\\cline{1-6}
\multirow{2}{*}{B} & baseline   & 0.757 & 136.9 & 0.846 & 64.9 \\\cline{2-6}
                         & TrustAL-NC & 0.758   & 118.0 & 0.840 & 60.0 \\\cline{1-6}
\multirow{2}{*}{C}   & baseline   & 0.769 & 123.9 & 0.851 & 60.0 \\\cline{2-6}
                         & TrustAL-NC & 0.769   & 114.2 & 0.844 & 59.0 \\\cline{1-6}
 \hline
 \noalign{\hrule height0.8pt}
 \end{tabular}
\caption{Average performance of TrustAL-NC using BERT with (A) CONF (B) CORESET and (C) BADGE on SST-2.} 
\label{table:sensitivity-bert}
\end{table}

==> figure_files/table-sensitivity-dev.tex <==
% \begin{figure*}[t!]\small
%     \begin{center}
%     \begin{tabular}{ccc}
%     \epsfig{file=acl-ijcnlp2021-templates/figure/conf_diversity_uncertainty_gray.pdf, width=51mm} & \epsfig{file=acl-ijcnlp2021-templates/figure/CORESET_diversity_uncertainty_gray.pdf, width=51mm} &
%     \epsfig{file=acl-ijcnlp2021-templates/figure/badge_diversity_uncertainty_gray.pdf, width=51mm} \\
%     (a) CONF & (b) CORESET & (c) BADGE \\
%     \end{tabular}
%     \end{center}
%     \caption{\textbf{Sensitivity analysis on TREC} (a) Varying the ratio of $D_{dev}$ (b) Varying the hyper parameter of KD (c) Varying the size of the budget $k$.}
%     \label{fig:rq4-senti}
% \end{figure*}


% \begin{table*}[t]\small
% \setlength\extrarowheight{3pt}
% \centering
%  \begin{tabular}{c c c c c c}
%  \hline
%  \noalign{\hrule height 0.8pt}
%  \multirow{2}{*}{} & &\multicolumn{2}{c}{\textbf{Stable}} &\multicolumn{2}{c}{\textbf{Saturated}}\\\cline{3-6}
%                   & &\textbf{acc.} & \textbf{CI} & \textbf{acc.} & \textbf{CI} \\
% \hline
% \noalign{\hrule height0.8pt}
% \multirow{3}{*}{Ratio of $D_{dev}$} & 0.5  & 0.794(\textcolor{red}{+0.038}) & 25.92(\textcolor{blue}{-6.07})  & 0.902(\textcolor{red}{+0.069}) & 14.06(\textcolor{blue}{-14.40}) \\\cline{2-6}
%                               & 1.0* & 0.796(\textcolor{red}{+0.017}) & 17.13(\textcolor{blue}{-4.61}) & 0.896(\textcolor{red}{+0.048}) & 14.08(\textcolor{blue}{-11.49}) \\\cline{2-6}
%                               & 2.0 & 0.794(\textcolor{red}{+0.05}) & 22.29(\textcolor{blue}{-7.24}) & 0.893(\textcolor{red}{+0.06}) & 14.52(\textcolor{blue}{-10.01}) \\\cline{1-6}
% \multirow{3}{*}{Size of budget $k$} & 0.02* & 0.796(\textcolor{red}{+0.017}) & 17.13(\textcolor{blue}{-4.61}) & 0.896(\textcolor{red}{+0.048}) & 14.08(\textcolor{blue}{-11.49}) \\\cline{2-6}
%                               & 0.04 & 0.787(\textcolor{blue}{-0.002}) & 16.78(\textcolor{blue}{-1.19}) & 0.911(\textcolor{red}{+0.040}) & 10.85(\textcolor{blue}{-10.76}) \\\cline{2-6}
%                               & 0.1 & 0.816(\textcolor{red}{+0.010}) & 10.98(\textcolor{blue}{-6.23}) & 0.897(\textcolor{blue}{-0.004}) & 13.21(\textcolor{blue}{-2.22}) \\\cline{1-6}
% \multirow{4}{*}{KD Loss Hyp.} & 0.3 & 0.794(\textcolor{red}{+0.015}) & 19.28(\textcolor{blue}{-2.47}) & 0.884(\textcolor{red}{+0.036}) & 17.53(\textcolor{blue}{-8.04}) \\\cline{2-6}
%                               & 0.75* & 0.796(\textcolor{red}{+0.017}) & 17.13(\textcolor{blue}{-4.61}) & 0.896(\textcolor{red}{+0.048}) & 14.08(\textcolor{blue}{-11.49}) \\\cline{2-6}
%                               & 1.5 & 0.792(\textcolor{red}{+0.013}) & 16.79(\textcolor{blue}{-4.96}) & 0.904(\textcolor{red}{+0.056}) & 10.73(\textcolor{blue}{-14.84}) \\\cline{2-6}
%                               & 10 & 0.797(\textcolor{red}{+0.018}) & 13.81(\textcolor{blue}{-7.94}) & 0.891(\textcolor{red}{+0.043}) & 10.66(\textcolor{blue}{-14.91}) \\\cline{2-6}
%                               & 20 & 0.788(\textcolor{red}{+0.010}) & 11.51(\textcolor{blue}{-10.23}) & 0.887(\textcolor{red}{+0.039}) & 10.33(\textcolor{blue}{-15.24}) \\\cline{1-6}
%  \hline
%  \noalign{\hrule height0.8pt}
%  \end{tabular}
% \caption{Performance of TrustAL-NC with BADGE on TREC for sensitivity analysis in stable learning stage and saturated learning stage. The colored numbers are the difference between BADGE with each hyper-parameter. The performance is the average performance of each phase. The hyper-parameter of the experiment on section ~\ref{sec:rq.1} are marked with *. The results with the other AL algorithms are in Appendix.} 
% \label{table:sensitivity-dev}
% \end{table*}


% \begin{figure*}[t!]\small
%     \begin{center}
%     \begin{tabular}{ccc}
%     \epsfig{file=acl-ijcnlp2021-templates/figure/conf_diversity_uncertainty_gray.pdf, width=51mm} & \epsfig{file=acl-ijcnlp2021-templates/figure/CORESET_diversity_uncertainty_gray.pdf, width=51mm} &
%     \epsfig{file=acl-ijcnlp2021-templates/figure/badge_diversity_uncertainty_gray.pdf, width=51mm} \\
%     (a) CONF & (b) CORESET & (c) BADGE \\
%     \end{tabular}
%     \end{center}
%     \caption{\textbf{Sensitivity analysis on TREC} (a) Varying the ratio of $D_{dev}$ (b) Varying the hyper parameter of KD (c) Varying the size of the budget $k$.}
%     \label{fig:rq4-senti}
% \end{figure*}


\begin{table*}[t]\small
\setlength\extrarowheight{3pt}
\centering
 \begin{tabular}{c c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{} & &\multicolumn{2}{c}{\textbf{Stable Learning Stage}} &\multicolumn{2}{c}{\textbf{Saturated Learning Stage}}\\\cline{3-6}
                   & &\textbf{accuracy} & \textbf{MCI} & \textbf{accuracy} & \textbf{MCI} \\
\hline
\noalign{\hrule height0.8pt}
\multirow{3}{*}{Ratio of $D_{dev}$} & 0.5  & 0.792(+0.037) & 22.47(-9.53)  & 0.897(+0.063) & 13.40(-14.90) \\\cline{2-6}
                              & 1.0* & 0.796(+0.017) & 17.13(-4.61) & 0.896(+0.048) & 14.08(-11.49) \\\cline{2-6}
                              & 2.0 & 0.791(+0.011) & 19.12(-5.13) & 0.889(+0.053) & 15.96(-14.32) \\\cline{1-6}
                              
\multirow{3}{*}{Size of budget $k$} & 0.02* & 0.796(+0.017) & 17.13(-4.61) & 0.896(+0.048) & 14.08(-11.49) \\\cline{2-6}
                              & 0.04 & 0.787(-0.002) & 16.78(-1.19) & 0.911(+0.040) & 10.84(-10.77) \\\cline{2-6}
                              & 0.1 & 0.816(+0.010) & 10.98(-6.23) & 0.897(-0.004) & 13.21(-2.00) \\\cline{1-6}
\multirow{5}{*}{$\alpha$ for $L_{KL}$} & 0.3 & 0.794(+0.015) & 19.28(-2.47) & 0.884(+0.036) & 17.53(-8.04) \\\cline{2-6}
                              & 0.75* & 0.796(+0.017) & 17.13(-4.61) & 0.896(+0.048) & 14.08(-11.49) \\\cline{2-6}
                              & 1.5 & 0.792(+0.013) & 16.79(-4.96) & 0.904(+0.056) & 10.73(-14.84) \\\cline{2-6}
                              & 10 & 0.797(+0.018) & 13.81(-7.94) & 0.891(+0.043) & 10.66(-14.91) \\\cline{2-6}
                              & 20 & 0.788(+0.010) & 11.51(-10.23) & 0.887(+0.039) & 10.33(-15.24) \\\cline{1-6}
 \hline
 \noalign{\hrule height0.8pt}
 \end{tabular}
\caption{Performance of TrustAL-NC with BADGE on TREC for robustness analysis. The colored numbers are the difference from BADGE for each hyperparameter (green: improvement, purple: deterioration). The performance is the average performance of each stage. The hyperparameter of the experiment on section~\ref{sec:new_rq_1} is marked with *. The results with other AL algorithms are in Appendix (Table~\ref{table:ap.sensitivity-nc-conf} and~\ref{table:ap.sensitivity-nc-coreset}).} 
\label{table:sensitivity-dev}
\end{table*}

==> figure_files/table-wangcc.tex <==
\begin{table}[t!]\small
\setlength\extrarowheight{3pt}
\centering
 \begin{tabular}{c l c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multicolumn{2}{c}{} & \textbf{TREC} & \textbf{Movie review}  & \textbf{SST-2} \\
\hline
\noalign{\hrule height0.8pt}
\multirow{4}{*}{A}    & baseline   & 0.726 & 0.637 & 0.686 \\\cline{2-5}
                         & Ensemble & 0.770 & 0.669 & 0.727 \\\cline{2-5}
                         & TrustAL-MC & 0.743 & 0.654 & 0.705 \\\cline{2-5}
                         & TrustAL-NC   & \textbf{0.774} & \textbf{0.676} & \textbf{0.730} \\\cline{1-5}
\multirow{4}{*}{B} & baseline & 0.727 & 0.627 & 0.697 \\\cline{2-5}
                         & Ensemble   & 0.777 & 0.658 & 0.724 \\\cline{2-5}
                         & TrustAL-MC & 0.753 & 0.654 & 0.707 \\\cline{2-5}
                         & TrustAL-NC   & \textbf{0.785} & \textbf{0.665} & \textbf{0.724} \\\cline{1-5}
\multirow{4}{*}{C}   & baseline   & 0.735 & 0.636 & 0.681 \\\cline{2-5}
                         & Ensemble   & 0.773 & 0.668 & 0.722 \\\cline{2-5}
                         & TrustAL-MC & 0.748 & 0.653 & 0.711 \\\cline{2-5}
                         & TrustAL-NC & \textbf{0.780} & \textbf{0.670} & \textbf{0.729} \\\cline{1-5}
 \hline
 \noalign{\hrule height0.8pt}
 \end{tabular}
\caption{Correct consistency of TrustAL-NC with (A) CONF (B) CORESET and (C) BADGE} 
\label{table:ap.wangcorrectconsistency}
\end{table}
